Bayesian Physics Informed Neural Networks for Linear Inverse problems

Inverse problems arise almost everywhere in science and engineering where we need to infer on a quantity from indirect observation. The cases of medical, biomedical, and industrial imaging systems are the typical examples. A very high overview of classification of the inverse problems method can be: i) Analytical, ii) Regularization, and iii) Bayesian inference methods. Even if there are straight links between them, we can say that the Bayesian inference based methods are the most powerful, as they give the possibility of accounting for prior knowledge and can account for errors and uncertainties in general. One of the main limitations stay in computational costs in particular for high dimensional imaging systems. Neural Networks (NN), and in particular Deep NNs (DNN), have been considered as a way to push farther this limit. Physics Informed Neural Networks (PINN) concept integrates physical laws with deep learning techniques to enhance the speed, accuracy and efficiency of the above mentioned problems. In this work, a new Bayesian framework for the concept of PINN (BPINN) is presented and discussed which includes the deterministic one if we use the Maximum A Posteriori (MAP) estimation framework. We consider two cases of supervised and unsupervised for training step, obtain the expressions of the posterior probability of the unknown variables, and deduce the posterior laws of the NN's parameters. We also discuss about the challenges of implementation of these methods in real applications.

==> arxiv/alphabet1.tex <==
% Document LaTeX based on Alphabet by Guy Lebesnerai
% Ali Mohammad-Djafari (janvier 2013)
% Objectif : Definitions for bold Math writing
%
% b pour bold italique : 		\ab \Ab
% v pour bold droit :    		\av \Av
% D pour droit :         		\aD \AD
% c pour cursif :					\Ac
% cb pour cursif bold:       		\Acb
% Grec italique: 				\alphab \Sigmab

% h pour \widehat:         		\ah \Ah \alphah \Sigmah
% t pour \widetilde:       		\at \At \alphat \Sigmat
% bt pour \widetilde\bold: 		\abt \Abt \alphabt \Sigmabt
% bh pour \widehat\bold:   		\abh \Abh \alphabh \Sigmabh

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
\typeout{\space}

%\RequirePackage{amsmath}
%\RequirePackage{xspace}
%\RequirePackage{oldgerm}		% 04.06.2003   Pour les alphabet Gauthiques

%-------------------------------------------
% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)
\def\bm#1{\mbox{\boldmath $#1$}}
%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative
\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}

% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras
\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}

% ALPHABET DROIT EN MATHS, taille adaptative
\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}

% ALPHABET GRAS DROIT, taille adaptative
\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}

% ALPHABET GREC GRAS italique, taille adaptative
\def\alphab{{\sbmm{\alpha}}\XS}
\def\betab{{\sbmm{\beta}}\XS}
\def\gammab{{\sbmm{\gamma}}\XS}      \def\Gammab{{\sbmm{\Gamma}}\XS}
\def\deltab{{\sbmm{\delta}}\XS}      \def\Deltab{{\sbmm{\Delta}}\XS}
\def\epsilonb{{\sbmm{\epsilon}}\XS}
\def\varepsilonb{{\sbmm{\varepsilon}}\XS}
\def\etab{{\sbmm{\eta}}\XS}
\def\thetab{{\sbmm{\theta}}\XS}      \def\Thetab{{\sbmm{\Theta}}\XS}
\def\varthetab{{\sbmm{\vartheta}}\XS}
\def\iotab{{\sbmm{\iota}}\XS}
\def\kappab{{\sbmm{\kappa}}\XS}
\def\varkappab{{\sbmm{\varkappa}}\XS}
\def\lambdab{{\sbmm{\lambda}}\XS}     \def\Lambdab{{\sbmm{\Lambda}}\XS}
\def\mub{{\sbmm{\mu}}\XS}
\def\nub{{\sbmm{\nu}}\XS}
\def\xib{{\sbmm{\xi}}\XS}         		\def\Xib{{\sbmm{\Xi}}\XS}
\def\pib{{\sbmm{\pi}}\XS}         		\def\Pib{{\sbmm{\Pi}}\XS}
\def\varpib{{\sbmm{\varpi}}\XS}
\def\rhob{{\sbmm{\rho}}\XS}
\def\varrhob{{\sbmm{\varrho}}\XS}
\def\sigmab{{\sbmm{\sigma}}\XS}      	\def\Sigmab{{\sbmm{\Sigma}}\XS}
\def\varsigmab{{\sbmm{\varsigma}}\XS}   \def\Varsigmab{{\sbmm{\Varsigma}}\XS}
\def\phib{{\sbmm{\phi}}\XS}        		\def\Phib{{\sbmm{\Phi}}\XS}
\def\varphib{{\sbmm{\varphi}}\XS}
\def\chib{{\sbmm{\chi}}\XS}
\def\psib{{\sbmm{\psi}}\XS}        		\def\Psib{{\sbmm{\Psi}}\XS}
\def\omegab{{\sbmm{\omega}}\XS}      	\def\Omegab{{\sbmm{\Omega}}\XS}
\def\taub{{\sbmm{\tau}}\XS}
\def\upsilonb{{\sbmm{\upsilon}}\XS}   	\def\Upsilonb{{\sbmm{\Upsilon}}\XS}
\def\zetab{{\sbmm{\zeta}}\XS}

%\widehat
\def\Ah{{\widehat{A}}\XS}  \def\ah{{\widehat{a}}\XS}
\def\Bh{{\widehat{B}}\XS}  \def\bh{{\widehat{b}}\XS}
\def\Ch{{\widehat{C}}\XS}  \def\ch{{\widehat{c}}\XS}
\def\Dh{{\widehat{D}}\XS}  \def\dh{{\widehat{d}}\XS}
\def\Eh{{\widehat{E}}\XS}  \def\eh{{\widehat{e}}\XS}
\def\Fh{{\widehat{F}}\XS}  \def\fh{{\widehat{f}}\XS}
\def\Gh{{\widehat{G}}\XS}  \def\gh{{\widehat{g}}\XS}
\def\Hh{{\widehat{H}}\XS}  \def\hh{{\widehat{h}}\XS}
\def\Ih{{\widehat{I}}\XS}  \def\ih{{\widehat{i}}\XS}
\def\Jh{{\widehat{J}}\XS}  \def\jh{{\widehat{j}}\XS}
\def\Kh{{\widehat{K}}\XS}  \def\kh{{\widehat{k}}\XS}
\def\Lh{{\widehat{L}}\XS}  \def\lh{{\widehat{l}}\XS}
\def\Mh{{\widehat{M}}\XS}  \def\mh{{\widehat{m}}\XS}
\def\Nh{{\widehat{N}}\XS}  \def\nh{{\widehat{n}}\XS}
\def\Oh{{\widehat{O}}\XS}  \def\oh{{\widehat{o}}\XS}
\def\Ph{{\widehat{P}}\XS}  \def\ph{{\widehat{p}}\XS}
\def\Qh{{\widehat{Q}}\XS}  \def\qh{{\widehat{q}}\XS}
\def\Rh{{\widehat{R}}\XS}  \def\rh{{\widehat{r}}\XS}
\def\Sh{{\widehat{S}}\XS}  \def\sh{{\widehat{s}}\XS}
\def\Th{{\widehat{T}}\XS}  \def\th{{\widehat{t}}\XS}
\def\Uh{{\widehat{U}}\XS}  \def\uh{{\widehat{u}}\XS}
\def\Vh{{\widehat{V}}\XS}  \def\vh{{\widehat{v}}\XS}
\def\Wh{{\widehat{W}}\XS}  \def\wh{{\widehat{w}}\XS}
\def\Xh{{\widehat{X}}\XS}  \def\xh{{\widehat{x}}\XS}
\def\Yh{{\widehat{Y}}\XS}  \def\yh{{\widehat{y}}\XS}
\def\Zh{{\widehat{Z}}\XS}  \def\zh{{\widehat{z}}\XS}

%\widetilde
%\def\At{{\widetilde{A}}\XS}  \def\at{{\widetilde{a}}\XS}
\def\Qt{{\widetilde{Q}}\XS}  \def\qt{{\widetilde{q}}\XS}
\def\Zt{{\widetilde{Z}}\XS}  \def\zt{{\widetilde{z}}\XS}

%\widetilde\bold
\def\Abt{{\widetilde{\Ab}}\XS}  \def\abt{{\widetilde{\ab}}\XS}
\def\Bbt{{\widetilde{\Bb}}\XS}  \def\bbt{{\widetilde{\bb}}\XS}
\def\Cbt{{\widetilde{\Cb}}\XS}  \def\cbt{{\widetilde{\cb}}\XS}
\def\Dbt{{\widetilde{\Db}}\XS}  \def\dbt{{\widetilde{\db}}\XS}
\def\Ebt{{\widetilde{\Eb}}\XS}  \def\ebt{{\widetilde{\eb}}\XS}
\def\Fbt{{\widetilde{\Fb}}\XS}  \def\fbt{{\widetilde{\fb}}\XS}
\def\Gbt{{\widetilde{\Gb}}\XS}  \def\gbt{{\widetilde{\gb}}\XS}
\def\Hbt{{\widetilde{\Hb}}\XS}  \def\hbt{{\widetilde{\hb}}\XS}
\def\Ibt{{\widetilde{\Ib}}\XS}  \def\ibt{{\widetilde{\ib}}\XS}
\def\Jbt{{\widetilde{\Jb}}\XS}  \def\jbt{{\widetilde{\jb}}\XS}
\def\Kbt{{\widetilde{\Kb}}\XS}  \def\kbt{{\widetilde{\kb}}\XS}
\def\Lbt{{\widetilde{\Lb}}\XS}  \def\lbt{{\widetilde{\lb}}\XS}
\def\Mbt{{\widetilde{\Mb}}\XS}  \def\mbt{{\widetilde{\mb}}\XS}
\def\Nbt{{\widetilde{\Nb}}\XS}  \def\nbt{{\widetilde{\nb}}\XS}
\def\Obt{{\widetilde{\Ob}}\XS}  \def\obt{{\widetilde{\ob}}\XS}
\def\Pbt{{\widetilde{\Pb}}\XS}  \def\pbt{{\widetilde{\pb}}\XS}
\def\Qbt{{\widetilde{\Qb}}\XS}  \def\qbt{{\widetilde{\qb}}\XS}
\def\Rbt{{\widetilde{\Rb}}\XS}  \def\rbt{{\widetilde{\rb}}\XS}
\def\Sbt{{\widetilde{\Sb}}\XS}  \def\sbt{{\widetilde{\sb}}\XS}
\def\Tbt{{\widetilde{\Tb}}\XS}  \def\tbt{{\widetilde{\tb}}\XS}
\def\Ubt{{\widetilde{\Ub}}\XS}  \def\ubt{{\widetilde{\ub}}\XS}
\def\Vbt{{\widetilde{\Vb}}\XS}  \def\vbt{{\widetilde{\vb}}\XS}
\def\Wbt{{\widetilde{\Wb}}\XS}  \def\wbt{{\widetilde{\wb}}\XS}
\def\Xbt{{\widetilde{\Xb}}\XS}  \def\xbt{{\widetilde{\xb}}\XS}
\def\Ybt{{\widetilde{\Yb}}\XS}  \def\ybt{{\widetilde{\yb}}\XS}
\def\Zbt{{\widetilde{\Zb}}\XS}  \def\zbt{{\widetilde{\zb}}\XS}

%\widehat\bold
\def\Abh{{\widehat{\Ab}}\XS}  \def\abh{{\widehat{\ab}}\XS}
\def\Bbh{{\widehat{\Bb}}\XS}  \def\bbh{{\widehat{\bb}}\XS}
\def\Cbh{{\widehat{\Cb}}\XS}  \def\cbh{{\widehat{\cb}}\XS}
\def\Dbh{{\widehat{\Db}}\XS}  \def\dbh{{\widehat{\db}}\XS}
\def\Ebh{{\widehat{\Eb}}\XS}  \def\ebh{{\widehat{\eb}}\XS}
\def\Fbh{{\widehat{\Fb}}\XS}  \def\fbh{{\widehat{\fb}}\XS}
\def\Gbh{{\widehat{\Gb}}\XS}  \def\gbh{{\widehat{\gb}}\XS}
\def\Hbh{{\widehat{\Hb}}\XS}  \def\hbh{{\widehat{\hb}}\XS}
\def\Ibh{{\widehat{\Ib}}\XS}  \def\ibh{{\widehat{\ib}}\XS}
\def\Jbh{{\widehat{\Jb}}\XS}  \def\jbh{{\widehat{\jb}}\XS}
\def\Kbh{{\widehat{\Kb}}\XS}  \def\kbh{{\widehat{\kb}}\XS}
\def\Lbh{{\widehat{\Lb}}\XS}  \def\lbh{{\widehat{\lb}}\XS}
\def\Mbh{{\widehat{\Mb}}\XS}  \def\mbh{{\widehat{\mb}}\XS}
\def\Nbh{{\widehat{\Nb}}\XS}  \def\nbh{{\widehat{\nb}}\XS}
\def\Obh{{\widehat{\Ob}}\XS}  \def\obh{{\widehat{\ob}}\XS}
\def\Pbh{{\widehat{\Pb}}\XS}  \def\pbh{{\widehat{\pb}}\XS}
\def\Qbh{{\widehat{\Qb}}\XS}  \def\qbh{{\widehat{\qb}}\XS}
\def\Rbh{{\widehat{\Rb}}\XS}  \def\rbh{{\widehat{\rb}}\XS}
\def\Sbh{{\widehat{\Sb}}\XS}  \def\sbh{{\widehat{\sb}}\XS}
\def\Tbh{{\widehat{\Tb}}\XS}  \def\tbh{{\widehat{\tb}}\XS}
\def\Ubh{{\widehat{\Ub}}\XS}  \def\ubh{{\widehat{\ub}}\XS}
\def\Vbh{{\widehat{\Vb}}\XS}  \def\vbh{{\widehat{\vb}}\XS}
\def\Wbh{{\widehat{\Wb}}\XS}  \def\wbh{{\widehat{\wb}}\XS}
\def\Xbh{{\widehat{\Xb}}\XS}  \def\xbh{{\widehat{\xb}}\XS}
\def\Ybh{{\widehat{\Yb}}\XS}  \def\ybh{{\widehat{\yb}}\XS}
\def\Zbh{{\widehat{\Zb}}\XS}  \def\zbh{{\widehat{\zb}}\XS}

%\widehat greek
\def\alphah{{\widehat{\alpha}}\XS}
\def\betah{{\widehat{\beta}}\XS}
\def\gammah{{\widehat{\gamma}}\XS}      \def\Gammah{{\widehat{\Gamma}}\XS}
\def\deltah{{\widehat{\delta}}\XS}      \def\Deltah{{\widehat{\Delta}}\XS}
\def\epsilonh{{\widehat{\epsilon}}\XS}
\def\varepsilonh{{\widehat{\varepsilon}}\XS}
\def\etah{{\widehat{\eta}}\XS}
\def\thetah{{\widehat{\theta}}\XS}      \def\Thetah{{\widehat{\Theta}}\XS}
\def\varthetah{{\widehat{\vartheta}}\XS}
\def\iotah{{\widehat{\iota}}\XS}
\def\kappah{{\widehat{\kappa}}\XS}
\def\varkappah{{\widehat{\varkappa}}\XS}
\def\lambdah{{\widehat{\lambda}}\XS}     \def\Lambdah{{\widehat{\Lambda}}\XS}
\def\muh{{\widehat{\mu}}\XS}
\def\nuh{{\widehat{\nu}}\XS}
\def\xih{{\widehat{\xi}}\XS}         		\def\Xih{{\widehat{\Xi}}\XS}
\def\pih{{\widehat{\pi}}\XS}         		\def\Pih{{\widehat{\Pi}}\XS}
\def\varpih{{\widehat{\varpi}}\XS}
\def\rhoh{{\widehat{\rho}}\XS}
\def\varrhoh{{\widehat{\varrho}}\XS}
\def\sigmah{{\widehat{\sigma}}\XS}      	\def\Sigmah{{\widehat{\Sigma}}\XS}
\def\varsigmah{{\widehat{\varsigma}}\XS}   \def\Varsigmah{{\widehat{\Varsigma}}\XS}
\def\phih{{\widehat{\phi}}\XS}        		\def\Phih{{\widehat{\Phi}}\XS}
\def\varphih{{\widehat{\varphi}}\XS}
\def\chih{{\widehat{\chi}}\XS}
\def\psih{{\widehat{\psi}}\XS}        		\def\Psih{{\widehat{\Psi}}\XS}
\def\omegah{{\widehat{\omega}}\XS}      	\def\Omegah{{\widehat{\Omega}}\XS}
\def\tauh{{\widehat{\tau}}\XS}
\def\upsilonh{{\widehat{\upsilon}}\XS}   	\def\Upsilonh{{\widehat{\Upsilon}}\XS}
\def\zetah{{\widehat{\zeta}}\XS}

%\widetilde greek
\def\alphat{{\widetilde{\alpha}}\XS}
\def\betat{{\widetilde{\beta}}\XS}
\def\gammat{{\widetilde{\gamma}}\XS}      \def\Gammat{{\widetilde{\Gamma}}\XS}
\def\deltat{{\widetilde{\delta}}\XS}      \def\Deltat{{\widetilde{\Delta}}\XS}
\def\epsilont{{\widetilde{\epsilon}}\XS}
\def\varepsilont{{\widetilde{\varepsilon}}\XS}
\def\etat{{\widetilde{\eta}}\XS}
\def\thetat{{\widetilde{\theta}}\XS}      \def\Thetat{{\widetilde{\Theta}}\XS}
\def\varthetat{{\widetilde{\vartheta}}\XS}
\def\iotat{{\widetilde{\iota}}\XS}
\def\kappat{{\widetilde{\kappa}}\XS}
\def\varkappat{{\widetilde{\varkappa}}\XS}
\def\lambdat{{\widetilde{\lambda}}\XS}     \def\Lambdat{{\widetilde{\Lambda}}\XS}
\def\mut{{\widetilde{\mu}}\XS}
\def\nut{{\widetilde{\nu}}\XS}
\def\xit{{\widetilde{\xi}}\XS}         		\def\Xit{{\widetilde{\Xi}}\XS}
\def\pit{{\widetilde{\pi}}\XS}         		\def\Pit{{\widetilde{\Pi}}\XS}
\def\varpit{{\widetilde{\varpi}}\XS}
\def\rhot{{\widetilde{\rho}}\XS}
\def\varrhot{{\widetilde{\varrho}}\XS}
\def\sigmat{{\widetilde{\sigma}}\XS}      	\def\Sigmat{{\widetilde{\Sigma}}\XS}
\def\varsigmat{{\widetilde{\varsigma}}\XS}   \def\Varsigmat{{\widetilde{\Varsigma}}\XS}
\def\phit{{\widetilde{\phi}}\XS}        		\def\Phit{{\widetilde{\Phi}}\XS}
\def\varphit{{\widetilde{\varphi}}\XS}
\def\chit{{\widetilde{\chi}}\XS}
\def\psit{{\widetilde{\psi}}\XS}        		\def\Psit{{\widetilde{\Psi}}\XS}
\def\omegat{{\widetilde{\omega}}\XS}      	\def\Omegat{{\widetilde{\Omega}}\XS}
\def\taut{{\widetilde{\tau}}\XS}
\def\upsilont{{\widetilde{\upsilon}}\XS}   	\def\Upsilont{{\widetilde{\Upsilon}}\XS}
\def\zetat{{\widetilde{\zeta}}\XS}

%\widehat\bold\greek
\def\alphabh{{\widehat{\alphab}}\XS}
\def\betabh{{\widehat{\betab}}\XS}
\def\gammabh{{\widehat{\gammab}}\XS}      \def\Gammabh{{\widehat{\Gammab}}\XS}
\def\deltabh{{\widehat{\deltab}}\XS}      \def\Deltabh{{\widehat{\Deltab}}\XS}
\def\epsilonbh{{\widehat{\epsilonb}}\XS}
\def\varepsilonbh{{\widehat{\varepsilonb}}\XS}
\def\etabh{{\widehat{\etab}}\XS}
\def\thetabh{{\widehat{\thetab}}\XS}      \def\Thetabh{{\widehat{\Thetab}}\XS}
\def\varthetabh{{\widehat{\varthetab}}\XS}
\def\iotabh{{\widehat{\iotab}}\XS}
\def\kappabh{{\widehat{\kappab}}\XS}
\def\varkappabh{{\widehat{\varkappab}}\XS}
\def\lambdabh{{\widehat{\lambdab}}\XS}     \def\Lambdabh{{\widehat{\Lambdab}}\XS}
\def\mubh{{\widehat{\mub}}\XS}
\def\nubh{{\widehat{\nub}}\XS}
\def\xibh{{\widehat{\xib}}\XS}         		\def\Xibh{{\widehat{\Xib}}\XS}
\def\pibh{{\widehat{\pib}}\XS}         		\def\Pibh{{\widehat{\Pib}}\XS}
\def\varpibh{{\widehat{\varpib}}\XS}
\def\rhobh{{\widehat{\rhob}}\XS}
\def\varrhobh{{\widehat{\varrhob}}\XS}
\def\sigmabh{{\widehat{\sigmab}}\XS}      	\def\Sigmabh{{\widehat{\Sigmab}}\XS}
\def\varsigmabh{{\widehat{\varsigmab}}\XS}   \def\Varsigmabh{{\widehat{\Varsigmab}}\XS}
\def\phibh{{\widehat{\phib}}\XS}        		\def\Phibh{{\widehat{\Phib}}\XS}
\def\varphibh{{\widehat{\varphib}}\XS}
\def\chibh{{\widehat{\chib}}\XS}
\def\psibh{{\widehat{\psib}}\XS}        		\def\Psibh{{\widehat{\Psib}}\XS}
\def\omegabh{{\widehat{\omegab}}\XS}      	\def\Omegabh{{\widehat{\Omegab}}\XS}
\def\taubh{{\widehat{\taub}}\XS}
\def\upsilonbh{{\widehat{\upsilonb}}\XS}   	\def\Upsilonbh{{\widehat{\Upsilonb}}\XS}
\def\zetabh{{\widehat{\zetab}}\XS}

%\widetilde\bold\greek
\def\alphabt{{\widetilde{\alphab}}\XS}
\def\betabt{{\widetilde{\betab}}\XS}
\def\gammabt{{\widetilde{\gammab}}\XS}      \def\Gammabt{{\widetilde{\Gammab}}\XS}
\def\deltabt{{\widetilde{\deltab}}\XS}      \def\Deltabt{{\widetilde{\Deltab}}\XS}
\def\epsilonbt{{\widetilde{\epsilonb}}\XS}
\def\varepsilonbt{{\widetilde{\varepsilonb}}\XS}
\def\etabt{{\widetilde{\etab}}\XS}
\def\thetabt{{\widetilde{\thetab}}\XS}      \def\Thetabt{{\widetilde{\Thetab}}\XS}
\def\varthetabt{{\widetilde{\varthetab}}\XS}
\def\iotabt{{\widetilde{\iotab}}\XS}
\def\kappabt{{\widetilde{\kappab}}\XS}
\def\varkappabt{{\widetilde{\varkappab}}\XS}
\def\lambdabt{{\widetilde{\lambdab}}\XS}     \def\Lambdabt{{\widetilde{\Lambdab}}\XS}
\def\mubt{{\widetilde{\mub}}\XS}
\def\nubt{{\widetilde{\nub}}\XS}
\def\xibt{{\widetilde{\xib}}\XS}         		\def\Xibt{{\widetilde{\Xib}}\XS}
\def\pibt{{\widetilde{\pib}}\XS}         		\def\Pibt{{\widetilde{\Pib}}\XS}
\def\varpibt{{\widetilde{\varpib}}\XS}
\def\rhobt{{\widetilde{\rhob}}\XS}
\def\varrhobt{{\widetilde{\varrhob}}\XS}
\def\sigmabt{{\widetilde{\sigmab}}\XS}      	\def\Sigmabt{{\widetilde{\Sigmab}}\XS}
\def\varsigmabt{{\widetilde{\varsigmab}}\XS}   \def\Varsigmabt{{\widetilde{\Varsigmab}}\XS}
\def\phibt{{\widetilde{\phib}}\XS}        		\def\Phibt{{\widetilde{\Phib}}\XS}
\def\varphibt{{\widetilde{\varphib}}\XS}
\def\chibt{{\widetilde{\chib}}\XS}
\def\psibt{{\widetilde{\psib}}\XS}        		\def\Psibt{{\widetilde{\Psib}}\XS}
\def\omegabt{{\widetilde{\omegab}}\XS}      	\def\Omegabt{{\widetilde{\Omegab}}\XS}
\def\taubt{{\widetilde{\taub}}\XS}
\def\upsilonbt{{\widetilde{\upsilonb}}\XS}   	\def\Upsilonbt{{\widetilde{\Upsilonb}}\XS}
\def\zetabt{{\widetilde{\zetab}}\XS}


==> arxiv/alphabet2.tex <==
% rbt pour \red\bold\widetilde: \rabt \rAbt \ralphabt \rSigmabt
% rbh pour \red\bold\widehat:   \rabh \rAbh \ralphahb \rSigmabh
% bbt pour \blue\bold\widetilde:\babt \bAbt
% bbh pour \blue\bold\widehat:  \babh \bAbh

\def\blue#1{{\color{blue}#1}}
\def\red#1{{\color{red}#1}} 
\def\green#1{{\color{green}#1}} 

%\red
\def\rH{{\red{H}}}  %\def\rh{{\red{h}}}
\def\rF{{\red{F}}}  %\def\rf{{\red{f}}}
\def\rZ{{\red{Z}}}  %\def\rz{{\red{z}}}
\def\rFb{{\red{\Fb}}}  \def\rfj{{\red{f_j}}}
\def\rZb{{\red{\Zb}}}  \def\rzj{{\red{z_j}}}
\def\rYb{{\red{\Yb}}}  \def\ryi{{\red{y_i}}}
\def\rtaue{{\red{\tau_\epsilon}}}  
\def\rtaub{{\red{\taub}}}
\def\rTaub{{\red{\Tb}}}
\def\rTaubt{{\red{\widetilde{\Tb}}}}
\def\rlambdat{{\red{\widetilde{\lambda}}}}

\def\rze{\red{z_{\epsilon}}}
\def\rzei{\red{z_{\epsilon_i}}}
\def\rzfj{\red{z_{f_j}}}
\def\rzbe{\red{\zb_{\epsilon}}}
\def\rzbf{\red{\zb_{f}}}
\def\alphaf{\alpha_f}
\def\betaf{\beta_f}

\def\rvzj{\red{{v_z}_j}}
\def\rmzj{\red{{m_z}_j}}
\def\rvjk{\red{{v_j}_k}}
\def\rmjk{\red{{m_j}_k}}
\def\ralphajk{\red{{\alpha_j}_k}}


%\blue
\def\bG{{\blue{G}}}  \def\bg{{\blue{g}}}

%\red\bold
\def\rAb{{\red{\Ab}}}  \def\rab{{\red{\ab}}}
\def\rBb{{\red{\Bb}}}  \def\rbb{{\red{\bb}}}
\def\rCb{{\red{\Cb}}}  \def\rcb{{\red{\cb}}}
\def\rDb{{\red{\Db}}}  \def\rdb{{\red{\db}}}
\def\rEb{{\red{\Eb}}}  \def\reb{{\red{\eb}}}
\def\rFb{{\red{\Fb}}}  \def\rfb{{\red{\fb}}}
\def\rGb{{\red{\Gb}}}  \def\rgb{{\red{\gb}}}
\def\rHb{{\red{\Hb}}}  \def\rhb{{\red{\hb}}}
\def\rIb{{\red{\Ib}}}  \def\rib{{\red{\ib}}}
\def\rJb{{\red{\Jb}}}  \def\rjb{{\red{\jb}}}
\def\rKb{{\red{\Kb}}}  \def\rkb{{\red{\kb}}}
\def\rLb{{\red{\Lb}}}  \def\rlb{{\red{\lb}}}
\def\rMb{{\red{\Mb}}}  \def\rmb{{\red{\mb}}}
\def\rNb{{\red{\Nb}}}  \def\rnb{{\red{\nb}}}
\def\rOb{{\red{\Ob}}}  \def\rob{{\red{\ob}}}
\def\rPb{{\red{\Pb}}}  \def\rpb{{\red{\pb}}}
\def\rQb{{\red{\Qb}}}  \def\rqb{{\red{\qb}}}
\def\rRb{{\red{\Rb}}}  \def\rrb{{\red{\rb}}}
\def\rSb{{\red{\Sb}}}  \def\rsb{{\red{\sb}}}
\def\rTb{{\red{\Tb}}}  \def\rtb{{\red{\tb}}}
\def\rUb{{\red{\Ub}}}  \def\rub{{\red{\ub}}}
\def\rVb{{\red{\Vb}}}  \def\rvb{{\red{\vb}}}
\def\rWb{{\red{\Wb}}}  \def\rwb{{\red{\wb}}}
\def\rXb{{\red{\Xb}}}  \def\rxb{{\red{\xb}}}
\def\rYb{{\red{\Yb}}}  \def\ryb{{\red{\yb}}}
\def\rZb{{\red{\Zb}}}  \def\rzb{{\red{\zb}}}

%\blue\bold
\def\bAb{{\blue{\Ab}}}  \def\bab{{\blue{\ab}}}
\def\bBb{{\blue{\Bb}}}  \def\bbb{{\blue{\bb}}}
\def\bCb{{\blue{\Cb}}}  \def\bcb{{\blue{\cb}}}
\def\bDb{{\blue{\Db}}}  \def\bdb{{\blue{\db}}}
\def\bEb{{\blue{\Eb}}}  \def\beb{{\blue{\eb}}}
\def\bFb{{\blue{\Fb}}}  \def\bfb{{\blue{\fb}}}
\def\bGb{{\blue{\Gb}}}  \def\bgb{{\blue{\gb}}}
\def\bHb{{\blue{\Hb}}}  \def\bhb{{\blue{\hb}}}
\def\bIb{{\blue{\Ib}}}  \def\bib{{\blue{\ib}}}
\def\bJb{{\blue{\Jb}}}  \def\bjb{{\blue{\jb}}}
\def\bKb{{\blue{\Kb}}}  \def\bkb{{\blue{\kb}}}
\def\bLb{{\blue{\Lb}}}  \def\blb{{\blue{\lb}}}
\def\bMb{{\blue{\Mb}}}  \def\bmb{{\blue{\mb}}}
\def\bNb{{\blue{\Nb}}}  \def\bnb{{\blue{\nb}}}
\def\bOb{{\blue{\Ob}}}  \def\bob{{\blue{\ob}}}
\def\bPb{{\blue{\Pb}}}  \def\bpb{{\blue{\pb}}}
\def\bQb{{\blue{\Qb}}}  \def\bqb{{\blue{\qb}}}
\def\bRb{{\blue{\Rb}}}  \def\brb{{\blue{\rb}}}
\def\bSb{{\blue{\Sb}}}  \def\bsb{{\blue{\sb}}}
\def\bTb{{\blue{\Tb}}}  \def\btb{{\blue{\tb}}}
\def\bUb{{\blue{\Ub}}}  \def\bub{{\blue{\ub}}}
\def\bVb{{\blue{\Vb}}}  \def\bvb{{\blue{\vb}}}
\def\bWb{{\blue{\Wb}}}  \def\bwb{{\blue{\wb}}}
\def\bXb{{\blue{\Xb}}}  \def\bxb{{\blue{\xb}}}
\def\bYb{{\blue{\Yb}}}  \def\byb{{\blue{\yb}}}
\def\bZb{{\blue{\Zb}}}  \def\bzb{{\blue{\zb}}}

%\red\widehat\bold
\def\rAbh{{\widehat{\rAb}}}  \def\rabh{{\widehat{\rab}}}
\def\rBbh{{\widehat{\rBb}}}  \def\rbbh{{\widehat{\rbb}}}
\def\rCbh{{\widehat{\rCb}}}  \def\rcbh{{\widehat{\rcb}}}
\def\rDbh{{\widehat{\rDb}}}  \def\rdbh{{\widehat{\rdb}}}
\def\rEbh{{\widehat{\rEb}}}  \def\rebh{{\widehat{\reb}}}
\def\rFbh{{\widehat{\rFb}}}  \def\rfbh{{\widehat{\rfb}}}
\def\rGbh{{\widehat{\rGb}}}  \def\rgbh{{\widehat{\rgb}}}
\def\rHbh{{\widehat{\rHb}}}  \def\rhbh{{\widehat{\rhb}}}
\def\rIbh{{\widehat{\rIb}}}  \def\ribh{{\widehat{\rib}}}
\def\rJbh{{\widehat{\rJb}}}  \def\rjbh{{\widehat{\rjb}}}
\def\rKbh{{\widehat{\rKb}}}  \def\rkbh{{\widehat{\rkb}}}
\def\rLbh{{\widehat{\rLb}}}  \def\rlbh{{\widehat{\rlb}}}
\def\rMbh{{\widehat{\rMb}}}  \def\rmbh{{\widehat{\rmb}}}
\def\rNbh{{\widehat{\rNb}}}  \def\rnbh{{\widehat{\rnb}}}
\def\rObh{{\widehat{\rOb}}}  \def\robh{{\widehat{\rob}}}
\def\rPbh{{\widehat{\rPb}}}  \def\rpbh{{\widehat{\rpb}}}
\def\rQbh{{\widehat{\rQb}}}  \def\rqbh{{\widehat{\rqb}}}
\def\rRbh{{\widehat{\rRb}}}  \def\rrbh{{\widehat{\rrb}}}
\def\rSbh{{\widehat{\rSb}}}  \def\rsbh{{\widehat{\rsb}}}
\def\rTbh{{\widehat{\rTb}}}  \def\rtbh{{\widehat{\rtb}}}
\def\rUbh{{\widehat{\rUb}}}  \def\rubh{{\widehat{\rub}}}
\def\rVbh{{\widehat{\rVb}}}  \def\rvbh{{\widehat{\rvb}}}
\def\rWbh{{\widehat{\rWb}}}  \def\rwbh{{\widehat{\rwb}}}
\def\rXbh{{\widehat{\rXb}}}  \def\rxbh{{\widehat{\rxb}}}
\def\rYbh{{\widehat{\rYb}}}  \def\rybh{{\widehat{\ryb}}}
\def\rZbh{{\widehat{\rZb}}}  \def\rzbh{{\widehat{\rzb}}}

%\red\widetilde\bold
\def\rAbt{{\widetilde{\rAb}}}  \def\rabt{{\widetilde{\rab}}}
\def\rBbt{{\widetilde{\rBb}}}  \def\rbbt{{\widetilde{\rbb}}}
\def\rCbt{{\widetilde{\rCb}}}  \def\rcbt{{\widetilde{\rcb}}}
\def\rDbt{{\widetilde{\rDb}}}  \def\rdbt{{\widetilde{\rdb}}}
\def\rEbt{{\widetilde{\rEb}}}  \def\rebt{{\widetilde{\reb}}}
\def\rFbt{{\widetilde{\rFb}}}  \def\rfbt{{\widetilde{\rfb}}}
\def\rGbt{{\widetilde{\rGb}}}  \def\rgbt{{\widetilde{\rgb}}}
\def\rHbt{{\widetilde{\rHb}}}  \def\rhbt{{\widetilde{\rhb}}}
\def\rIbt{{\widetilde{\rIb}}}  \def\ribt{{\widetilde{\rib}}}
\def\rJbt{{\widetilde{\rJb}}}  \def\rjbt{{\widetilde{\rjb}}}
\def\rKbt{{\widetilde{\rKb}}}  \def\rkbt{{\widetilde{\rkb}}}
\def\rLbt{{\widetilde{\rLb}}}  \def\rlbt{{\widetilde{\rlb}}}
\def\rMbt{{\widetilde{\rMb}}}  \def\rmbt{{\widetilde{\rmb}}}
\def\rNbt{{\widetilde{\rNb}}}  \def\rnbt{{\widetilde{\rnb}}}
\def\rObt{{\widetilde{\rOb}}}  \def\robt{{\widetilde{\rob}}}
\def\rPbt{{\widetilde{\rPb}}}  \def\rpbt{{\widetilde{\rpb}}}
\def\rQbt{{\widetilde{\rQb}}}  \def\rqbt{{\widetilde{\rqb}}}
\def\rRbt{{\widetilde{\rRb}}}  \def\rrbt{{\widetilde{\rrb}}}
\def\rSbt{{\widetilde{\rSb}}}  \def\rsbt{{\widetilde{\rsb}}}
\def\rTbt{{\widetilde{\rTb}}}  \def\rtbt{{\widetilde{\rtb}}}
\def\rUbt{{\widetilde{\rUb}}}  \def\rubt{{\widetilde{\rub}}}
\def\rVbt{{\widetilde{\rVb}}}  \def\rvbt{{\widetilde{\rvb}}}
\def\rWbt{{\widetilde{\rWb}}}  \def\rwbt{{\widetilde{\rwb}}}
\def\rXbt{{\widetilde{\rXb}}}  \def\rxbt{{\widetilde{\rxb}}}
\def\rYbt{{\widetilde{\rYb}}}  \def\rybt{{\widetilde{\ryb}}}
\def\rZbt{{\widetilde{\rZb}}}  \def\rzbt{{\widetilde{\rzb}}}

%\red\bold\greek
\def\ralphab{{\red{\alphab}}}
\def\rbetab{{\red{\betab}}}
\def\rgammab{{\red{\gammab}}}      \def\rGammab{{\red{\Gammab}}}
\def\rdeltab{{\red{\deltab}}}      \def\rDeltab{{\red{\Deltab}}}
\def\repsilonb{{\red{\epsilonb}}}
\def\rvarepsilonb{{\red{\varepsilonb}}}
\def\retab{{\red{\etab}}}
\def\rthetab{{\red{\thetab}}}      \def\rThetab{{\red{\Thetab}}}
\def\rvarthetab{{\red{\varthetab}}}
\def\riotab{{\red{\iotab}}}
\def\rkappab{{\red{\kappab}}}
\def\rvarkappab{{\red{\varkappab}}}
\def\rlambdab{{\red{\lambdab}}}     \def\rLambdab{{\red{\Lambdab}}}
\def\rmub{{\red{\mub}}}
\def\rnub{{\red{\nub}}}
\def\rxib{{\red{\xib}}}         		\def\rXib{{\red{\Xib}}}
\def\rpib{{\red{\pib}}}         		\def\rPib{{\red{\Pib}}}
\def\rvarpib{{\red{\varpib}}}
\def\rrhob{{\red{\rhob}}}
\def\rvarrhob{{\red{\varrhob}}}
\def\rsigmab{{\red{\sigmab}}}      	\def\rSigmab{{\red{\Sigmab}}}
\def\rvarsigmab{{\red{\varsigmab}}}   \def\rVarsigmab{{\red{\Varsigmab}}}
\def\rphib{{\red{\phib}}}        		\def\rPhib{{\red{\Phib}}}
\def\rvarphib{{\red{\varphib}}}
\def\rchib{{\red{\chib}}}
\def\rpsib{{\red{\psib}}}        		\def\rPsib{{\red{\Psib}}}
\def\romegab{{\red{\omegab}}}      	\def\rOmegab{{\red{\Omegab}}}
\def\rtaub{{\red{\taub}}}
\def\rupsilonb{{\red{\upsilonb}}}   	\def\rUpsilonb{{\red{\Upsilonb}}}
\def\rzetab{{\red{\zetab}}}

%\red\widehat\bold\greek
\def\ralphabh{{\red{\alphabh}}}
\def\rbetabh{{\red{\betabh}}}
\def\rgammabh{{\red{\gammabh}}}      \def\rGammabh{{\red{\Gammabh}}}
\def\rdeltabh{{\red{\deltabh}}}      \def\rDeltabh{{\red{\Deltabh}}}
\def\repsilonbh{{\red{\epsilonbh}}}
\def\rvarepsilonbh{{\red{\varepsilonbh}}}
\def\retabh{{\red{\etabh}}}
\def\rthetabh{{\red{\thetabh}}}      \def\rThetabh{{\red{\Thetabh}}}
\def\rvarthetabh{{\red{\varthetabh}}}
\def\riotabh{{\red{\iotabh}}}
\def\rkappabh{{\red{\kappabh}}}
\def\rvarkappabh{{\red{\varkappabh}}}
\def\rlambdabh{{\red{\lambdabh}}}     \def\rLambdabh{{\red{\Lambdabh}}}
\def\rmubh{{\red{\mubh}}}
\def\rnubh{{\red{\nubh}}}
\def\rxibh{{\red{\xibh}}}         		\def\rXibh{{\red{\Xibh}}}
\def\rpibh{{\red{\pibh}}}         		\def\rPibh{{\red{\Pibh}}}
\def\rvarpibh{{\red{\varpibh}}}
\def\rrhobh{{\red{\rhobh}}}
\def\rvarrhobh{{\red{\varrhobh}}}
\def\rsigmabh{{\red{\sigmabh}}}      	\def\rSigmabh{{\red{\Sigmabh}}}
\def\rvarsigmabh{{\red{\varsigmabh}}}   \def\rVarsigmabh{{\red{\Varsigmabh}}}
\def\rphibh{{\red{\phibh}}}        		\def\rPhibh{{\red{\Phibh}}}
\def\rvarphibh{{\red{\varphibh}}}
\def\rchibh{{\red{\chibh}}}
\def\rpsibh{{\red{\psibh}}}        		\def\rPsibh{{\red{\Psibh}}}
\def\romegabh{{\red{\omegabh}}}      	\def\rOmegabh{{\red{\Omegabh}}}
\def\rtaubh{{\red{\taubh}}}
\def\rupsilonbh{{\red{\upsilonbh}}}   	\def\rUpsilonbh{{\red{\Upsilonbh}}}
\def\rzetabh{{\red{\zetabh}}}

%\red\widetilde\bold\greek
\def\ralphabt{{\red{\alphabt}}}
\def\rbetabt{{\red{\betabt}}}
\def\rgammabt{{\red{\gammabt}}}      \def\rGammabt{{\red{\Gammabt}}}
\def\rdeltabt{{\red{\deltabt}}}      \def\rDeltabt{{\red{\Deltabt}}}
\def\repsilonbt{{\red{\epsilonbt}}}
\def\rvarepsilonbt{{\red{\varepsilonbt}}}
\def\retabt{{\red{\etabt}}}
\def\rthetabt{{\red{\thetabt}}}      \def\rThetabt{{\red{\Thetabt}}}
\def\rvarthetabt{{\red{\varthetabt}}}
\def\riotabt{{\red{\iotabt}}}
\def\rkappabt{{\red{\kappabt}}}
\def\rvarkappabt{{\red{\varkappabt}}}
\def\rlambdabt{{\red{\lambdabt}}}     \def\rLambdabt{{\red{\Lambdabt}}}
\def\rmubt{{\red{\mubt}}}
\def\rnubt{{\red{\nubt}}}
\def\rxibt{{\red{\xibt}}}         		\def\rXibt{{\red{\Xibt}}}
\def\rpibt{{\red{\pibt}}}         		\def\rPibt{{\red{\Pibt}}}
\def\rvarpibt{{\red{\varpibt}}}
\def\rrhobt{{\red{\rhobt}}}
\def\rvarrhobt{{\red{\varrhobt}}}
\def\rsigmabt{{\red{\sigmabt}}}      	\def\rSigmabt{{\red{\Sigmabt}}}
\def\rvarsigmabt{{\red{\varsigmabt}}}   \def\rVarsigmabt{{\red{\Varsigmabt}}}
\def\rphibt{{\red{\phibt}}}        		\def\rPhibt{{\red{\Phibt}}}
\def\rvarphibt{{\red{\varphibt}}}
\def\rchibt{{\red{\chibt}}}
\def\rpsibt{{\red{\psibt}}}        		\def\rPsibt{{\red{\Psibt}}}
\def\romegabt{{\red{\omegabt}}}      	\def\rOmegabt{{\red{\Omegabt}}}
\def\rtaubt{{\red{\taubt}}}
\def\rupsilonbt{{\red{\upsilonbt}}}   	\def\rUpsilonbt{{\red{\Upsilonbt}}}
\def\rzetabt{{\red{\zetabt}}}

%\red\widetilde\greek
\def\ralphat{{\red{\alphat}}}
\def\rbetat{{\red{\betat}}}
\def\rgammat{{\red{\gammat}}}      \def\rGammat{{\red{\Gammat}}}
\def\rdeltat{{\red{\deltat}}}      \def\rDeltat{{\red{\Deltat}}}
\def\repsilont{{\red{\epsilont}}}
\def\rvarepsilont{{\red{\varepsilont}}}
\def\retat{{\red{\etat}}}
\def\rthetat{{\red{\thetat}}}      \def\rThetat{{\red{\Thetat}}}
\def\rvarthetat{{\red{\varthetat}}}
\def\riotat{{\red{\iotat}}}
\def\rkappat{{\red{\kappat}}}
\def\rvarkappat{{\red{\varkappat}}}
\def\rlambdat{{\red{\lambdat}}}     \def\rLambdat{{\red{\Lambdat}}}
\def\rmut{{\red{\mut}}}
\def\rnut{{\red{\nut}}}
\def\rxit{{\red{\xit}}}         		\def\rXit{{\red{\Xit}}}
\def\rpit{{\red{\pit}}}         		\def\rPit{{\red{\Pit}}}
\def\rvarpit{{\red{\varpit}}}
\def\rrhot{{\red{\rhot}}}
\def\rvarrhot{{\red{\varrhot}}}
\def\rsigmat{{\red{\sigmat}}}      	\def\rSigmat{{\red{\Sigmat}}}
\def\rvarsigmat{{\red{\varsigmat}}}   \def\rVarsigmat{{\red{\Varsigmat}}}
\def\rphit{{\red{\phit}}}        		\def\rPhit{{\red{\Phit}}}
\def\rvarphit{{\red{\varphit}}}
\def\rchit{{\red{\chit}}}
\def\rpsit{{\red{\psit}}}        		\def\rPsit{{\red{\Psit}}}
\def\romegat{{\red{\omegat}}}      	\def\rOmegat{{\red{\Omegat}}}
\def\rtaut{{\red{\taut}}}
\def\rupsilont{{\red{\upsilont}}}   	\def\rUpsilont{{\red{\Upsilont}}}
\def\rzetat{{\red{\zetat}}}


==> arxiv/macros_gpi.tex <==
% macros_gpi.tex
\def\bdoc{\begin{document}}             \def\edoc{\end{document}}
\def\babs{\begin{abstract}}             \def\eabs{\end{abstract}}
\def\bcc{\begin{center}}                \def\ecc{\end{center}}
\def\ben{\begin{enumerate}}             \def\een{\end{enumerate}}
\def\bit{\begin{itemize}}               \def\eit{\end{itemize}}
\def\bpic{\begin{picture}}              \def\epic{\end{picture}}
\def\barr{\begin{array}}                \def\earr{\end{array}}
\def\btabu{\begin{tabular}}             \def\etabu{\end{tabular}}
\def\bcc{\begin{center}}                \def\ecc{\end{center}}
\def\bfig{\begin{figure}}               \def\efig{\end{figure}}
\def\bver{\begin{verb}}					\def\ever{\end{verb}}
\def\bbib{\begin{thebibliography}{999}}	\def\ebib{\end{thebibliography}}

\def\beq{\begin{equation}}				\def\eeq{\end{equation}}
\def\bmult{\begin{multline}}			\def\emult{\end{multline}}
\def\balign{\begin{align}}				\def\ealign{\end{align}}
\def\beqn{\begin{eqnarray}}             \def\eeqn{\end{eqnarray}}
\def\beqnx{\begin{eqnarray*}}           \def\eeqnx{\end{eqnarray*}}

\def\bm#1{\mbox{\boldmath $#1$}}
%\def\bm#1{\mbox{$\boldmath{#1}$}}
%\def\bm#1{\mathbf{#1}}

%Numbers
\def\zerob{{\bm 0}}
\def\oneb{{\bm 1}}

%Small letters
\def\ab{{\bm a}}
\def\bb{{\bm b}}
\def\cb{{\bm c}}
\def\db{{\bm d}}
\def\eb{{\bm e}}
\def\fb{{\bm f}}
\def\gb{{\bm g}}
\def\hb{{\bm h}}
\def\ib{{\bm i}}
\def\jb{{\bm j}}
\def\kb{{\bm k}}
\def\lb{{\bm l}}
\def\mb{{\bm m}}
\def\nb{{\bm n}}
\def\ob{{\bm o}}
\def\pb{{\bm p}}
\def\qb{{\bm q}}
\def\rb{{\bm r}}
\def\sb{{\bm s}}
\def\tb{{\bm t}}
\def\ub{{\bm u}}
\def\vb{{\bm v}}
\def\wb{{\bm w}}
\def\xb{{\bm x}}
\def\yb{{\bm y}}
\def\zb{{\bm z}}

%Capital letters
\def\Ab{{\bm A}}
\def\Bb{{\bm B}}
\def\Cb{{\bm C}}
\def\Db{{\bm D}}
\def\Eb{{\bm E}}
\def\Fb{{\bm F}}
\def\Gb{{\bm G}}
\def\Hb{{\bm H}}
\def\Ib{{\bm I}}
\def\Jb{{\bm J}}
\def\Kb{{\bm K}}
\def\Lb{{\bm L}}
\def\Mb{{\bm M}}
\def\Nb{{\bm N}}
\def\Ob{{\bm O}}
\def\Pb{{\bm P}}
\def\Qb{{\bm Q}}
\def\Rb{{\bm R}}
\def\Sb{{\bm S}}
\def\Tb{{\bm T}}
\def\Ub{{\bm U}}
\def\Vb{{\bm V}}
\def\Wb{{\bm W}}
\def\Xb{{\bm X}}
\def\Yb{{\bm Y}}
\def\Zb{{\bm Z}}

%Small Greek letters
\def\alphab{\bm{\alpha}}
\def\betab{\bm{\beta}}
\def\deltab{\bm{\delta}}
\def\etab{\bm{\eta}}
\def\epsilonb{\bm{\epsilon}}
\def\gammab{\bm{\gamma}}
\def\omegab{\bm{\omega}}
\def\etab{\bm{\eta}}
\def\thetab{\bm{\theta}}
\def\xib{\bm{\xi}}
\def\lambdab{\bm{\lambda}}
\def\taub{\bm{\tau}}
\def\phib{\bm{\phi}}
\def\mub{\bm{\mu}}
\def\psib{\bm{\psi}}
\def\chib{\bm{\chi}}
\def\sigmab{\bm{\sigma}}

%Capital Greek letters
\def\Deltab{\bm{\Delta}}
\def\Lambdab{\bm{\Lambda}}
\def\Phib{\bm{\Phi}}
\def\Psib{\bm{\Psi}}
\def\Sigmab{\bm{\Sigma}}

%Caligraphic capital letters
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}

\def\disp#1{\displaystyle{#1}}

%Arrows
\def\ra{\rightarrow}
\def\la{\leftarrow}
\def\da{\downarrow}
\def\ua{\uparrow}

\def\Ra{\Rightarrow}
\def\La{\Leftarrow}
\def\Da{\Downarrow}
\def\Ua{\Uparrow}

\def\lra{\longrightarrow}
\def\lla{\longleftarrow}
\def\Lra{\Longrightarrow}
\def\Lla{\longleftarrow}

\def\lrarr{\leftrightarrow}
\def\Lrarr{\Leftrightarrow}
\def\udarr{\updownarrow}
\def\Uparr{\Updownarrow}

%INTEGRALES
\def\d#1{\,\mbox{d} #1}
\def\iii{\int_{-\infty}^{+\infty}}
\def\izi{\int_{0}^{\infty}}
\def\izpi{\int_{0}^{\pi}}
\def\izdpi{\int_{0}^{2\pi}}
\def\intd{\int\kern-.8em\int}
\def\intt{\int\kern-.8em\int\kern-.8em\int}
\def\intg{\int\kern-1.1em\int}

%widehat
\def\wh{\widehat}
\def\xh{\widehat{x}}
\def\thetah{\widehat{\theta}}
\def\betah{\widehat{\beta}}

\def\xbh{\widehat{\xb}}
\def\ybh{\widehat{\yb}}
\def\thetabh{\widehat{\thetab}}
\def\etabh{\widehat{\etab}}
\def\betabh{\widehat{\betab}}

% iterations
\def\xbhk{\widehat{\xb}^{k}}
\def\thetahk{\widehat{\theta}^{k}}
\def\betahk{\widehat{\beta}^{k}}

\def\xbhkp{\widehat{\xb}^{k+1}}
\def\thetahkp{\widehat{\theta}^{k+1}}
\def\betahkp{\widehat{\beta}^{k+1}}

\def\thetabhk{\widehat{\thetab}^{k}}
\def\betabhk{\widehat{\betab}^{k}}

\def\thetabhkp{\widehat{\thetab}^{k+1}}
\def\betabhkp{\widehat{\betab}^{k+1}}

\def\thetamin{\theta_{\mbox{\tiny min}}}
\def\thetamax{\theta_{\mbox{\tiny max}}}
\def\betamin{\beta_{\mbox{\tiny min}}}
\def\betamax{\beta_{\mbox{\tiny max}}}

% functions with one parameter
\def\expf#1{\exp\left[ {#1} \right]}

\def\argmax#1#2{\arg\max_{#1}\left\{ #2 \right\}}
\def\argmin#1#2{\arg\min_{#1}\left\{ #2 \right\}}

\def\Prob#1{\mbox{Pr}\left\{#1\right\}}
\def\var#1{\mbox{Var}\left\{#1\right\}}
\def\cov#1{\mbox{Cov}\left\{#1\right\}}
\def\corr#1{\mbox{Corr}\left\{#1\right\}}
%\def\trace#1{\mbox{Tr}\left\{#1\right\}}
\def\rang#1{\mbox{rang}\left\{#1\right\}}
\def\det#1{\mbox{d\'et}\left\{#1\right\}}

\def\gbu{\underline{\gb}}
\def\fbu{\underline{\fb}}
\def\zbu{\underline{\zb}}
\def\epsilonbu{\underline{\epsilonb}}
\def\thetabu{\underline{\thetab}}

\def\ve{{v_{\epsilon}}}
\def\sigmae{{\sigma_{\epsilon}}}
\def\Sigmae{{\Sigmab_{\epsilonb}}}
\def\Sigmaf{{\Sigmab_{\fb}}}
\def\Sigmag{{\Sigmab_{\gb}}}

\def\fbuh{\widehat{\fbu}}
\def\zbuh{\widehat{\fbu}}
\def\thetabuh{\widehat{\thetabu}}

\def\fbh{\widehat{\fb}}
\def\Pbh{\widehat{\Pb}}
\def\Sigmabh{\widehat{\Sigmab}}
\def\Abh{\widehat{\Ab}}
\def\Bbh{\widehat{\Bb}}
\def\thetabh{\widehat{\thetab}}
\def\Rbe{\Rb_{\epsilon}}
\def\Rbeh{\widehat{\Rbe}}

\def\Rjk{{R_j}_k}
\def\fbik{{\fb_i}_k}
\def\fbjk{{\fb_j}_k}

\def\mik{{m_i}_k}
\def\sigmaik{{\sigma_i^2}_k}
\def\Sigmaik{{\Sigmab_i}_k}
\def\alphaik{{\alpha_i}_k}
\def\betaik{{\beta_i}_k}

\def\muik{{\mu_i}_k}
\def\vik{{v_i}_k}

\def\mjk{{m_j}_k}
\def\sigmajk{{\sigma_j^2}_k}
\def\Sigmajk{{\Sigmab_j}_k}
\def\alphajk{{\alpha_j}_k}
\def\betajk{{\beta_j}_k}

\def\mujk{{\mu_j}_k}
\def\vjk{{v_j}_k}
\def\njk{{n_j}_k}

\def\alphae{\alpha_{\epsilon}}
\def\betae{\beta_{\epsilon}}
\def\alphaez{\alpha_{\epsilon_0}}
\def\betaez{\beta_{\epsilon_0}}
\def\alphaei{\alpha_{\epsilon_i}}
\def\betaei{\beta_{\epsilon_i}}
\def\alphaeiz{\alpha_{\epsilon_{i_0}}}
\def\betaeiz{\beta_{\epsilon_{i-0}}}

\def\mbz{{{\mb}_z}}
\def\Sigmabz{{{\Sigmab}_z}}
\def\diag#1{\mbox{diag}\left[#1\right]}

\def\sigmah{\widehat{\sigma}}
\def\fh{\widehat{f}}
\def\sigmaz{\sigma_z}

\def\sumi{\sum_{i=1}^{M} }
\def\sumj{\sum_{j=1}^{N} }
\def\lambdah{\wh{\lambda}}
\def\lambdabh{\wh{\lambdab}}

\def\det#1{\hbox{det}\left(#1\right)}
\def\defined{\,\shortstack{$\triangle$\\ =}\,}

\def\zmat{\left[\matrix{0}\right]}
\def\det#1{\hbox{det}(#1)}
\def\th{\widehat{t}}
\def\xh{\widehat{x}}
\def\lambdah{\widehat{\lambda}}
\def\muh{\widehat{\mu}}
\def\sigmah{\widehat{\sigma}}
\def\rhoh{\widehat{\rho}}
\def\betah{\widehat{\beta}}
\def\alphah{\widehat{\alpha}}
\def\tauh{\widehat{\tau}}

\def\tbh{\widehat{\tb}}
\def\mubh{\widehat{\mub}}
\def\sigmabh{\widehat{\sigmab}}
\def\rhobh{\widehat{\rhob}}
\def\oneb{\mbox{\bf 1}}

\def\bm#1{\mbox{\boldmath $#1$}}
\def\zerob{{\bf 0}}
\def\oneb{{\bf 1}}
\def\intg{\int\kern-1.1em\int}
\def\expf#1{\exp\left[ {#1} \right]}

\def\gbu{\underline{\gb}}
\def\fbu{\underline{\fb}}
\def\zbu{\underline{\zb}}
\def\epsilonbu{\underline{\epsilonb}}
\def\uthetab{\underline{\thetab}}

\def\sigmae{{\sigma_{\epsilon}}}
\def\Sigmae{{\Sigma_{\epsilonb}}}
\def\Sigmabe{{\Sigmab_{\epsilonb}}}
\def\Sigmaf{{\Sigmab_{\fb}}}
\def\Sigmag{{\Sigmab_{\gb}}}

\def\fbuh{\widehat{\fbu}}
\def\zbuh{\widehat{\fbu}}
\def\uthetabh{\widehat{\uthetab}}

\def\fbh{\widehat{\fb}}
\def\Sigmabh{\widehat{\Sigmab}}
\def\Abh{\widehat{\Ab}}
\def\thetabh{\widehat{\thetab}}

\def\Rjk{{R_j}_k}
\def\fbik{{\fb_i}_k}
\def\fbjk{{\fb_j}_k}

\def\mik{{m_i}_k}
\def\sigmaik{{\sigma_i^2}_k}
\def\Sigmaik{{\Sigmab_i}_k}
\def\alphaik{{\alpha_i}_k}
\def\betaik{{\beta_i}_k}

\def\muik{{\mu_i}_k}
\def\vik{{v_i}_k}

\def\mjk{{m_j}_k}
\def\sigmajk{{\sigma_j^2}_k}
\def\Sigmajk{{\Sigmab_j}_k}
\def\alphajk{{\alpha_j}_k}
\def\betajk{{\beta_j}_k}

\def\mujk{{\mu_j}_k}
\def\vjk{{v_j}_k}
\def\njk{{n_j}_k}

\def\mbz{{{\mb}_z}}
\def\Sigmabz{{{\Sigmab}_z}}

\def\vect{\mbox{vect}}
\def\lra{\longrightarrow}

\def\gir{g_i(\rb)}
\def\fjr{f_j(\rb)}
\def\zjr{z_j(\rb)}
\def\epsilonir{\epsilon_i(\rb)}
\def\gbr{\gb(\rb)}
\def\fbr{\fb(\rb)}
\def\zbr{\zb(\rb)}
\def\epsilonbr{\epsilonb(\rb)}
\def\fbhr{\fbh(\rb)}
\def\Sigmabhr{\Sigmabh(\rb)}

\def\mbzr{\mb_{z(\rb)}}
\def\Sigmabzr{\Sigmab_{z(\rb)}}
\def\Sigmagbzr{{\Sigmab_g}_{z(\rb)}}

\def\mjzjr#1{{m_{#1}}_{z_{#1}(\rb)}}
\def\sigmajzjr#1{{\sigma_{#1}}_{z_{#1}(\rb)}}

\def\Beta{B}
\def\Betab{\bm{\Beta}}
\def\Betabe{\bm{\Beta}_{\epsilonb}}

\def\fh{\widehat{f}}
\def\sigmah{\widehat{\sigma}}
\def\sigmaei{\sigma_{\epsilon_i}^2}


\def\thetah{\widehat{\theta}}
\def\sigmah{\widehat{\sigma}}

\def\Ftxm{\widetilde{F}_{X}(x_-)}
\def\Ftxp{\widetilde{F}_{X}(x_+)}

\def\NU{{\cal V}}

\def\tFx{\widetilde{F}_{X}}

\def\Fx{F_{X}(x)}
\def\fx{f_{X}(x)}

\def\Fxv{F_{X}(x)}
\def\fxv{f_{X}(x)}

\def\Fxi{{F}_{X_i}(x_i)}
\def\fxi{{f}_{X_i}(x_i)}

\def\Gnu{G_{\NU}(\nu)}
\def\gnu{g_{\NU}(\nu)}

\def\Fnu{F_{\NU}(\nu)}
\def\fnu{f_{\NU}(\nu)}

\def\Finnu#1{F^{-1}_{\NU}(#1)}

\def\Gnua#1{G_{\NU}(#1)}
\def\Gnub#1{G_{\NU}^{-1}(#1)}
\def\Gnuh{G_{\NU}^{-1}(1/2)}

\def\Ftx{\widetilde{F}_{X}(x)}
\def\ftx{\widetilde{f}_{X}(x)}

\def\Ftxi{\widetilde{F}_{X_i}(x_i)}
\def\ftxi{\widetilde{f}_{X_i}(x_i)}

\def\Ftxv{\widetilde{F}_{X}(x)}
\def\FtX#1{\widetilde{F}_{X}(#1)}
\def\ftxv{\widetilde{f}_{X}(x)}

\def\fxnu{f_{X|\NU}(x|\nu)}
\def\fxNU{f_{X|\NU}(x|\NU)}
\def\FxNU{F_{X|\NU}(x|\NU)}

\def\fxNUtheta{f_{X|\NU,\theta}(x|\NU,\theta)}
\def\FxNUtheta{F_{X|\NU,\theta}(x|\NU,\theta)}

\def\Fxnu{F_{X|\NU}(x|\nu)}
\def\Fxnui#1{F_{X|\NU}(x|\nu_#1)}

\def\FxN#1{F_{X|\NU}(#1)}
\def\FxNU{F_{X|\NU}(x|\NU)}
\def\Fxnun#1{F_{X|\NU}(x|#1)}
\def\Fxinun#1{F_{X_i|\NU}(x_i|#1)}
\def\fxnu{f_{X|\NU}(x|\nu)}
\def\fxNU{f_{X|\NU}(x|\NU)}

\def\Fxvnu{F_{X|\NU}(x|\nu)}
\def\Fxvnun#1{F_{X|\NU}(x|#1)}
\def\FxvNU{F_{X|\NU}(x|\NU)}

\def\FXvnu{F_{X|\NU}}

\def\fxvnu{f_{X|\NU}(x|\nu)}
\def\fxvNU{f_{X|\NU}(x|\NU)}


\def\FXvNU#1{{F}_{X|\NU}(#1|\NU)}
\def\FXvn#1{{F}_{X|\NU}(x|#1)}

\def\Fxtheta{F_{X|\theta}(x|\theta)}
\def\fxtheta{f_{X|\theta}(x|\theta)}

\def\Fxvtheta{F_{X|\theta}(x|\theta)}
\def\fxvtheta{f_{X|\theta}(x|\theta)}

\def\Ftxtheta{\widetilde{F}_{X|\theta}(x|\theta)}
\def\ftxtheta{\widetilde{f}_{X|\theta}(x|\theta)}

\def\Ftxvtheta{\widetilde{F}_{X|\theta}(x|\theta)}
\def\ftxvtheta{\widetilde{f}_{X|\theta}(x|\theta)}

\def\Fxnutheta{F_{X|\NU,\theta}(x|\nu,\theta)}
\def\fxnutheta{f_{X|\NU,\theta}(x|\nu,\theta)}

\def\ftheta{f_{\Theta}(\theta)}
\def\fthetaxnuz{f_{\Theta|X,\nu_0}(\theta|x,\nu_0)}
\def\fthetax{f_{\Theta|X}(\theta|x)}

\def\Fxvnutheta{F_{X|\NU,\theta}(x|\nu,\theta)}
\def\FxvNUtheta{F_{X|\NU,\theta}(x|\NU,\theta)}
\def\fxvnutheta{f_{X|\NU,\theta}(x|\nu,\theta)}
\def\Ftxvnutheta{\widetilde{F}_{X|\theta}(x|\theta)}
\def\ftxvnutheta{\widetilde{f}_{X|\theta}(x|\theta)}

%\def\Ftxvm{\widetilde{F}_{X}(x_-)}
%\def\Ftxvp{\widetilde{F}_{X}(x_+)}
\def\FxvNUm{F_{X|\NU}(x_-|\NU)}
\def\FxvNUp{F_{X|\NU}(x_+|\NU)}

\def\Fxinu{F_{X_i|\NU}(x_i|\nu)}
\def\fxinu{f_{X_i|\NU}(x_i|\nu)}

\def\Ftxi{\widetilde{F}_{X_i}(x_i)}
\def\ftxi{\widetilde{f}_{X_i}(x_i)}

\def\fxitheta{f_{X_i|\theta}(x_i|\theta)}
\def\ftxitheta{\widetilde{f}_{X_i|\theta}(x_i|\theta)}

\def\thetah{\widehat{\theta}}
\def\thetat{\widetilde{\theta}}

%\def\Lnuxv{L_{\nu|X}(\nu|x)}
\def\lnuxv{l_{\nu|X}(\nu|x)}

\def\Lnuxva#1{L_{\nu|X}(#1 | x)}
\def\lnuxva#1{l_{\nu|X}(#1 | x)}

\def\Prob#1{\mbox{P}\left(#1\right)}

\def\lthetaxvnuz{l(\theta)}

\def\lthetaxvnuz{l_{\theta|x,\nu_0}(\theta | x,\nu_0)}
\def\fxnuztheta{f_{X|\nu_0,\theta}(x | \nu_0,\theta)}
\def\fxinuztheta{f_{X|\nu_0,\theta}(x_i | \nu_0,\theta)}
\def\fxvtheta{f_{X|\theta}(x | \theta)}
\def\lthetaxv{l_{\theta|X}(\theta | x)}
\def\ltthetaxv{\widetilde{l}_{\theta|X}(\theta | x)}

\def\ltheta{l(\theta )}
\def\lttheta{\widetilde{l}(\theta)}
\def\Lnu{L(\nu )}
\def\Lnui#1{L(\nu_#1)}
\def\Linu{L_i(\nu )}
\def\Linu{L_i(\nu )}
\def\LNU{L(\NU )}
\def\Lin#1{L^{-1}(#1)}
\def\L#1{L(#1)}
\def\Li#1{L_i(#1)}
\def\FNU#1{F_\NU(#1)}
\def\FinNU#1{F^{-1}_\NU(#1)}

\def\ftthetax{\tilde{f}_{\Theta|X}(\theta|x)}
\def\ER{R}

\def\Ndd#1#2#3{{\cal N}\left( #1 ;~ #2, #3 \right)}
\def\Cdd#1#2#3{{\cal C}\left( #1 ;~ #2, #3 \right)}
\def\Sdd#1#2#3#4{{\cal S}\left( #1 ;~ #2, #3, #4 \right)}
\def\Edd#1#2{{\cal E}\left( #1 ;~ #2 \right)}
\def\DEdd#1#2{{\cal DE}\left( #1 ;~ #2 \right)}
\def\Gdd#1#2#3{{\cal G}\left( #1 ;~ #2, #3 \right)}
\def\IGdd#1#2#3{{\cal IG}\left( #1 ;~ #2, #3 \right)}


\def\Xwr{X(\omega,\rb)}
\def\xwr{x(\omega,\rb)}

\def\muzw{\mu_{z}(\omega)}
\def\muzwr{\mu_{z(\rb)}(\omega)}
\def\szw{\sigma_{z}^2(\omega)}
\def\szwr{\sigma_{z(\rb)}^2(\omega)}
\def\pzw{p_{z}(\omega)}
\def\pzwr{p_{z(\rb)}(\omega)}

\def\hszw{\widehat{\sigma_{z}^2}(\omega)}
\def\hmuzw{\widehat{\mu}_{z}(\omega)}
\def\hpzw{\widehat{p}_{z}(\omega)}

\def\muzwrl{\mu_{z(\rb)}(\omega-l)}

\def\pxwrcz{p\left(\xwr ~|~ z\right)}
\def\pxwr{p\left(\xwr\right)}

\def\Xbw{\Xb(\omega)}
\def\xbw{\xb(\omega)}
\def\uXb{\underline{\Xb}}
\def\uxb{\underline{\xb}}
\def\pxbw{p(\xbw)}
\def\puxb{p(\uxb)}
\def\pzb{P(\zb)}

\def\Szw{S_z(\omega)}
\def\mubw{\mub(\omega)}

\def\Srw{S_{\rb}(\omega)}
\def\Swr{S_{\omega}(\rb)}
\def\Sbw{\Sb(\omega)}
\def\sbw{\sb(\omega)}
\def\Sbr{\Sb(\rb)}
\def\mubw{\mub(\omega)}
\def\cov#1{\mbox{cov}[#1]}

\def\pdf{\emph{pdf}}
\def\pmf{\emph{pmf}}
\def\dpdx#1#2{\frac{\partial #1}{\partial #2}}

\def\REM#1{}

\def\XXwr{X(\omega,\rb)}
\def\xxwr{x(\omega,\rb)}

\def\Xwr{X_{\omega}(\rb)}
\def\xwr{x_{\omega}(\rb)}
\def\Xrw{X_{\rb}(\omega)}
\def\xrw{x_{\rb}(\omega)}

\def\Ywr{Y_{\omega}(\rb)}
\def\ywr{y_{\omega}(\rb)}
\def\Yrw{Y_{\rb}(\omega)}
\def\yrw{y_{\rb}(\omega)}

\def\Ewr{E_{\omega}(\rb)}
\def\ewr{\epsilon_{\omega}(\rb)}
\def\Erw{E_{\rb}(\omega)}
\def\erw{\epsilon_{\rb}(\omega)}

\def\Xbr{\Xb(\rb)}
\def\xbr{\xb(\rb)}
\def\Xbw{\Xb(\omega)}
\def\xbw{\xb(\omega)}

\def\uXb{\underline{\Xb}}
\def\uxb{\underline{\xb}}
\def\uXbz{\underline{\Xb}_z}
\def\uxbz{\underline{\xb}_z}

\def\uthetab{\underline{\thetab}}
\def\uthetabz{\underline{\thetab}_z}

\def\Ywr{Y_{\omega}(\rb)}
\def\ywr{y_{\omega}(\rb)}
\def\Yrw{Y_{\rb}(\omega)}
\def\yrw{y_{\rb}(\omega)}
\def\Ybr{\Yb(\rb)}
\def\ybr{\yb(\rb)}
\def\Ybw{\Yb(\omega)}
\def\ybw{\yb(\omega)}
\def\uYb{\underline{\Yb}}
\def\uyb{\underline{\yb}}
\def\uYbz{\underline{\Yb}_z}
\def\uybz{\underline{\yb}_z}

\def\Ewr{E_{\omega}(\rb)}
\def\ewr{\epsilon_{\omega}(\rb)}
\def\Erw{E_{\rb}(\omega)}
\def\erw{\epsilon_{\rb}(\omega)}
\def\Ebr{Eb(\rb)}
\def\ebr{\epsilonb(\rb)}
\def\Ebw{Eb(\omega)}
\def\ebw{\epsilonb(\omega)}
\def\uEb{\underline{\Eb}}

\def\Erwp{E_{\rb}(\omega')}
\def\Xrwp{X_{\rb}(\omega')}

\def\xwmr{x_{\omega-1}(\rb)}
\def\muzwm{\mu_{z}(\omega-1)}

\def\rhoz{\rho_z}
\def\sez{\sigma_{\eta_z}^2}

\def\xwrp{x_{\omega}(\rb')}
\def\xrwp{x_{\rb}(\omega')}
\def\xwpr{x_{\omega'}(\rb)}
\def\xwprp{x_{\omega'}(\rb')}
\def\Xwrp{x_{\omega}(\rb')}
\def\Xwrp{X_{\omega}(\rb')}
\def\Xwpr{X_{\omega'}(\rb)}
\def\Xwprp{X_{\omega'}(\rb')}

\def\sigmaed{\sigmae^2}
\def\sigmaew{\sigmae(\omega)}
\def\sigmaedw{\sigmaed(\omega)}


\def\Sigmabe{\Sigmab_{\epsilon}}
\def\sigmabh{\widehat{\Sigmab}}
\def\xbh{\widehat{\xb}}
\def\zbh{\widehat{\zb}}
\def\qbh{\widehat{\qb}}
\def\sbh{\widehat{\sb}}

\def\espx#1#2{\mbox{E}_{#1}\left\{#2\right\}}
\def\esp#1{\mbox{E}\left\{#1\right\}}
\def\d#1{\mbox{~d}#1}

\def\Tr#1{\mbox{Tr}\left[#1\right]}

\def\pmatrix#1{\left[\barr{ccccccccccccccc} #1 \earr\right]}
\def\Bf{\bm{B}}
\def\gbh{\widehat{\gb}}
\def\dbh{\widehat{\db}}
\def\Tr#1{\mbox{Tr}\left[#1\right]}
\def\Cov#1{\mbox{Cov}\left[#1\right]}
\def\iid{i.i.d.~}

\def\cro#1{\left[#1\right]}
\def\acc#1{\left\{#1\right\}}
\def\aprio{\emph{a priori~}}
\def\apost{\emph{a posteriori~}}
\def\hbh{\widehat{\hb}}
\def\qh{\widehat{q}}
\def\fbt{\widetilde{\fb}}
\def\thetabt{\widetilde{\thetab}}


\def\mubt{\widetilde{\mub}}
\def\Sigmabt{\widetilde{\Sigmab}}
\def\qt{\widetilde{q}}
\def\vt{\widetilde{v}}
\def\zt{\widetilde{z}}
\def\Dbt{\widetilde{\Db}}
\def\alphat{\widetilde{\alpha}}
\def\betat{\widetilde{\beta}}
\def\abt{\widetilde{\ab}}
\def\ajt{\widetilde{a}_j}
\def\taut{\widetilde{\tau}}
\def\mut{\widetilde{\mu}}
\def\Zbt{\widetilde{\Zb}}
\def\Abt{\widetilde{\Ab}}
\def\zbt{\widetilde{\zb}}

\def\bloca#1#2#3{
\begin{picture}(50,50)
  \put(32,42){\makebox(0,0){#1}}
  \put(25,50){\vector(0,-1){20}}
  \put(0,10){\framebox(50,20){#2}}
  \put(0,0){\makebox(50,0){#3}}  
\end{picture}
}


\def\ugb{\underline{\gb}}
\def\fbh{\widehat{\fb}}
\def\zbh{\widehat{\zb}}
\def\qbh{\widehat{\qb}}
\def\thetabh{\widehat{\thetab}}
\def\Pbh{\widehat{\Pb}}

\def\sigmae{\sigma_{\epsilon}}
\def\REM#1{}
\def\fh{\widehat{f}}
\def\zh{\widehat{z}}
\def\disp{\displaystyle}
\def\oneb{{\boldmath{1}}}
\def\zerob{{\boldmath{0}}}
\def\d#1{\; \mbox{d} #1}
\def\expf#1{\exp\left\{#1\right\}}
\def\esp#1{\mbox{E}\left\{#1\right\}}
\def\lra{\longrightarrow}

\def\bslide#1{\begin{frame}{\Large\bf #1}}
\def\eslide{\end{frame}}

\def\inversions#1#2#3{
\begin{picture}(100,40)
  \put(0,15){\makebox(15,0){#1}}
  \put(20,15){\vector(1,0){10}}
  \put(30,7){\framebox(40,15){#2}}
  \put(70,15){\vector(1,0){10}}
  \put(85,15){\makebox(15,0){#3}}
\end{picture}
}

% colors
\def\blue#1{{\color{blue}#1}}
\def\red#1{{\color{red}#1}}
\def\green#1{{\color{green}#1}}

\def\rfb{\red{\fb}}
\def\bgb{\blue{\gb}}
\def\rfbh{\red{\widehat{\fb}}}
\def\rfbt{\red{\widetilde{\fb}}}
\def\rzbt{\red{\widetilde{\zb}}}
\def\rqb{\red{\qb}}
\def\rqbh{\red{\widehat{\qb}}}
\def\rzb{\red{\zb}}
\def\rzbh{\red{\widehat{\zb}}}
\def\rthetab{\red{\thetab}}
\def\retab{\red{\etab}}
\def\rthetabh{\red{\widehat{\thetab}}}
\def\rthetabt{\red{\widetilde{\thetab}}}
\def\retabt{\red{\widetilde{\etab}}}
\def\ralphabt{\red{\widetilde{\alphab}}}

\def\ugb{\underline{\gb}}
\def\fbh{\widehat{\fb}}
\def\zbh{\widehat{\zb}}
\def\qbh{\widehat{\qb}}
\def\thetabh{\widehat{\thetab}}
\def\Pbh{\widehat{\Pb}}

\def\UP#1{\uppercase{#1}}
\def\sca#1{\uppercase{#1}}


\def\sigmae{\sigma_{\epsilon}}
\def\REM#1{}
\def\fh{\widehat{f}}
\def\zh{\widehat{z}}
\def\disp{\displaystyle}
\def\oneb{{\boldmath{1}}}
\def\zerob{{\boldmath{0}}}
\def\d#1{\; \mbox{d} #1}
\def\expf#1{\exp\left\{#1\right\}}
\def\esp#1{\mbox{E}\left\{#1\right\}}
\def\lra{\longrightarrow}


\def\rfb{\red{\fb}}
\def\rFb{\red{\Fb}}
\def\bgb{\blue{\gb}}
\def\rfbh{\red{\widehat{\fb}}}
\def\rqb{\red{\qb}}
\def\rqbh{\red{\widehat{\qb}}}
\def\rzb{\red{\zb}}
\def\rzbh{\red{\widehat{\zb}}}
\def\rthetab{\red{\thetab}}
\def\ralphab{\red{\alphab}}
\def\rbetab{\red{\betab}}
\def\rthetabh{\red{\widehat{\thetab}}}
\def\ralphabh{\red{\widehat{\alphaab}}}
\def\rSigmab{\red{\Sigmab}}
\def\rSigmabe{\red{\Sigmabe}}


\def\rz{\red{z}}
\def\rzh{\red{\widehat{z}}}

\def\rab{\red{\ab}}
\def\rabh{\red{\widehat{\ab}}}
\def\rAb{\red{\Ab}}
\def\rAbh{\red{\widehat{\Ab}}}
\def\rBb{\red{\Bb}}
\def\rBbh{\red{\widehat{\Bb}}}
\def\rPbh{\red{\widehat{\Pb}}}
\def\rub{\red{\ub}}
\def\rubh{\red{\widehat{\ub}}}

\def\rVb{\red{\Vb}}
\def\rVbh{\widehat{\rVb}}
\def\rVbt{\widetilde{\rVb}}

\def\rvb{\red{\vb}}
\def\rvbh{\widehat{\rvb}}
\def\rvbt{\widetilde{\rvb}}

\def\bfb{\blue{\fb}}
\def\bFb{\blue{\Fb}}

\def\rfi{\red{f}_i}
\def\rfj{\red{f}_j}
\def\ruj{\red{u}_j}
\def\raj{\red{a}_j}
\def\rzj{\red{z}_j}
\def\rvj{\red{v}_j}
\def\rtau{\red{\tau}}
\def\rtauj{\red{\tau_j}}
\def\rtaub{\red{\taub}}
\def\rtauh{\widehat{\rtau}}
\def\rtaujh{\widehat{\rtauj}}
\def\rtaubh{\widehat{\rtaub}}
\def\rve{\red{v_{\epsilon}}}
\def\rv{\red{v}}

\def\rfjh{\red{\widehat{f}}_j}
\def\rujh{\red{\widehat{u}}_j}
\def\rajh{\red{\widehat{a}}_j}
\def\rzjh{\red{\widehat{z}}_j}
\def\rvjh{\red{\widehat{v}}_j}

\def\ralpha{\red{\alpha}}
\def\rbeta{\red{\beta}}
\def\rtheta{\red{\theta}}

\def\rlambda{\red{\lambda}}
\def\ralphah{\widehat{\ralpha}}
\def\rbetah{\widehat{\rbeta}}
\def\rthetah{\widehat{\rtheta}}
\def\rlambdah{\widehat{\rlambda}}

\def\ubh{\widehat{\ub}}


\def\rve{\red{v_{\epsilon}}}
\def\alphae{\alpha_{\epsilon_0}}
\def\betae{\beta_{\epsilon_0}}
\def\alphajh{\widehat{\alpha}_j}
\def\betajh{\widehat{\beta}_j}
\def\alphaeh{\widehat{\alpha}_{\epsilon_0}}
\def\betaeh{\widehat{\beta}_{\epsilon_0}}


\def\rqb{\red{\qb}}
\def\rqbh{\red{\widehat{\qb}}}
\def\rzb{\red{\zb}}
\def\rZb{\red{\Zb}}
\def\rab{\red{\ab}}
\def\rAb{\red{\Ab}}
\def\rvb{\red{\vb}}
\def\rmb{\red{\mb}}
\def\rzbh{\red{\widehat{\zb}}}
\def\rvbh{\red{\widehat{\vb}}}
\def\rmbh{\red{\widehat{\mb}}}
\def\rthetab{\red{\thetab}}
\def\rthetabh{\red{\widehat{\thetab}}}
\def\rfbh{\widehat{\rfb}}
\def\rhb{\red{\hb}}
\def\rhbh{\widehat{\rhb}}
\def\rthetai{\red{\theta}_i}
\def\rthetab{\red{\thetab}}
\def\rfjm{\red{f}_{j-1}}
\def\rfim{\red{f}_{i-1}}

\def\muh{\widehat{\mu}}
\def\vh{\widehat{v}}

\def\rSigmabh{\red{\Sigmabh}}
\def\rVbh{\red{\Vbh}}
\def\Fbh{\red{\Fb}}
\def\rFbh{\red{\Fbh}}

\def\Sigmabeh{\widehat{\Sigmabe}}
\def\rSigmabeh{\widehat{\red{\Sigmabe}}}


\def\rf{\red{f}}
\def\bg{\blue{g}}
\def\rF{\red{F}}
\def\bG{\blue{G}}

\def\sumk{\sum_{k=1}^K}
\def\suml{\sum_{l=1}^L}
\def\sumn{\sum_{n=1}^N}
\def\sumj{\sum_{j=1}^J}
\def\sumi{\sum_{i=1}^I}

\def\nub{\bm{\nu}}
\def\rak{\red{a_k}}
\def\rbk{\red{b_k}}
\def\rck{\red{c_k}}
\def\rtk{\red{t_k}}
\def\rvk{\red{v_k}}
\def\rnuk{\red{\nu_k}}
\def\rnuz{\red{\nu_0}}
\def\rphik{\red{\phi_k}}
\def\rnub{\red{\nub}}
\def\rtb{\red{\tb}}
\def\rphib{\red{\phib}}
\def\rfn{\red{f_n}}
\def\rtn{\red{t_n}}
\def\rvn{\red{v_n}}

\def\rve{\red{v_\epsilon}}
\def\rvf{\red{v_f}}
\def\rveh{\red{\widehat{v}_\epsilon}}
\def\rvfh{\red{\widehat{v}_f}}

\def\rnu{\red{\nu}}
\def\rphi{\red{\phi}}
\def\rbl{\red{b_l}}
\def\rbb{\red{\bb}}

\def\modela{\tt\setlength{\unitlength}{0.92pt}
\begin{picture}(250,106)
\thinlines    \put(-5,105){$\Nc(t|\red{t_1,v_1})$}
              \put(35,100){\vector(1,0){25}}
              \put(60,95){\framebox(37,16){\red{$a_1$}}}
			  \multiput(77,72)(0,7){3}{\circle*{4}}
              \put(-5,65){$\Nc(t|\red{t_k,v_k})$}
              \put(35,59){\vector(1,0){25}}
              \put(60,51){\framebox(37,16){\red{$a_k$}}}
              \multiput(77,32)(0,7){3}{\circle*{4}}              
              \put(-5,23){$\Nc(t|\red{t_K,v_K})$}
              \put(60,10){\framebox(37,16){\red{$a_K$}}}
              \put(35,18){\vector(1,0){25}}

              \put(98,103){\vector(1,-1){38}}
              \put(98,59){\vector(1,0){39}}
              \put(98,17){\vector(1,1){38}}

              \put(150,60){\circle{24}}
              \put(146,57){$\Large+$}
              \put(165,75){$g_{\rthetab}(t)$}
              \put(164,60){\vector(1,0){33}}
              
              \put(212,85){$\epsilon(t)$}
              \put(210,95){\vector(0,-1){20}}
              \put(211,60){\circle{24}}
              \put(207,58){$\Large+$}
              
              \put(225,66){$g(t)$}
              \put(225,60){\vector(1,0){20}}
\end{picture}
}

\def\modelb{\tt\setlength{\unitlength}{0.92pt}
\begin{picture}(250,106)
\thinlines    \put(-5,105){$\delta(t-\red{t_1})$}
              \put(0,100){\vector(1,0){37}}
              \put(38,95){\framebox(60,16){$\red{a_1} \Nc(t|0,\red{v_1})$}}
			  \multiput(77,72)(0,7){3}{\circle*{4}}
              \put(-5,65){$\delta(t-\red{t_k})$}
              \put(0,59){\vector(1,0){37}}
              \put(38,51){\framebox(60,16){$\red{a_k} \Nc(t|0,\red{v_k})$}}
              \multiput(77,32)(0,7){3}{\circle*{4}}              
              \put(-5,23){$\delta(t-\red{t_K})$}
              \put(38,10){\framebox(60,16){$\red{a_K} \Nc(t|0,\red{v_K})$}}
              \put(0,18){\vector(1,0){37}}

              \put(98,103){\vector(1,-1){38}}
              \put(98,59){\vector(1,0){39}}
              \put(98,17){\vector(1,1){38}}

              \put(150,60){\circle{24}}
              \put(146,57){$\Large+$}
              \put(165,75){$g_{\rthetab}(t)$}
              \put(164,60){\vector(1,0){33}}
              
              \put(212,85){$\epsilon(t)$}
              \put(210,95){\vector(0,-1){20}}
              \put(211,60){\circle{24}}
              \put(207,58){$\Large+$}
              
              \put(225,66){$g(t)$}
              \put(225,60){\vector(1,0){20}}
\end{picture}
}

\def\modelc{\tt\setlength{\unitlength}{0.92pt}
\begin{picture}(250,106)
\thinlines    \put(-5,105){$\delta(t-\red{t_1})$}
              \put(0,100){\vector(1,0){37}}
              \put(38,95){\framebox(40,16){$\red{a_1}$}}
			  \multiput(57,72)(0,7){3}{\circle*{4}}
              \put(-5,65){$\delta(t-\red{t_k})$}
              \put(0,59){\vector(1,0){37}}
              \put(38,51){\framebox(40,16){$\red{a_k}$}}
              \multiput(57,32)(0,7){3}{\circle*{4}}              
              \put(-5,23){$\delta(t-\red{t_K})$}
              \put(38,10){\framebox(40,16){$\red{a_K}$}}
              \put(0,18){\vector(1,0){37}}

              \put(78,103){\vector(1,-1){38}}
              \put(78,59){\vector(1,0){39}}
              \put(78,17){\vector(1,1){38}}

              \put(130,60){\circle{24}}
              \put(126,57){$\Large+$}
              \put(144,60){\vector(1,0){10}}
              \put(154,52){\framebox(50,16){$\Nc(t|0,v)$}}
              
              \put(205,75){$g_{\rthetab}(t)$}
              \put(204,60){\vector(1,0){33}}
              
              \put(252,85){$\epsilon(t)$}
              \put(250,95){\vector(0,-1){20}}
              \put(251,60){\circle{24}}
              \put(247,58){$\Large+$}
              
              \put(265,66){$g(t)$}
              \put(265,60){\vector(1,0){20}}
\end{picture}
}

\def\modeld{\tt\setlength{\unitlength}{0.92pt}
\begin{picture}(250,106)
\thinlines    \put(20,70){$s(t)=\sum_k \rak \delta(t-\red{t_k})$}
              \put(105,60){\vector(1,0){50}}
              \put(154,52){\framebox(50,16){$\Nc(t|0,v)$}}
              
              \put(205,75){$g_{\rthetab}(t)$}
              \put(204,60){\vector(1,0){33}}
              
              \put(252,85){$\epsilon(t)$}
              \put(250,95){\vector(0,-1){20}}
              \put(251,60){\circle{24}}
              \put(247,58){$\Large+$}
              
              \put(265,66){$g(t)$}
              \put(265,60){\vector(1,0){20}}
              \put(0,20){\siga}
\end{picture}
}

\def\siga{\setlength{\unitlength}{0.46pt}
\begin{picture}(290,108)
\thinlines    \put(10,26){\vector(1,0){260}}
              \put(16,12){\vector(0,1){88}}
              \put(48,27){\vector(0,1){34}}
              \put(79,27){\vector(0,1){54}}
              %\put(102,27){\vector(0,1){31}}
              \put(130,27){\vector(0,1){46}}
              \put(188,26){\vector(0,1){40}}
              \put(262,14){$t$}
              %\put(22,90){$s(t)$}
              \put(182,16){$\red{t_K}$}
              \put(195,63){$\red{a_K}$}
              \put(125,15){$\red{t_k}$}
              \put(137,68){$\red{a_k}$}
              \put(75,14){$\red{t_2}$}
              \put(84,73){$\red{a_2}$}
              \put(43,15){$\red{t_1}$}
              \put(54,56){$\red{a_1}$}
              \multiput(150,46)(8,0){3}{\circle*{4}}
\end{picture}
}

\def\modele{\tt\setlength{\unitlength}{0.92pt}
\begin{picture}(250,106)
\thinlines    \put(20,70){$s(t)=\sum_n \rfn \delta(t-n\Delta t)$}
              \put(105,60){\vector(1,0){50}}
              \put(154,52){\framebox(50,16){$\Nc(t|0,v)$}}
              
              \put(205,75){$g_{\rfb}(t)$}
              \put(204,60){\vector(1,0){33}}
              
              \put(252,85){$\epsilon(t)$}
              \put(250,95){\vector(0,-1){20}}
              \put(251,60){\circle{24}}
              \put(247,58){$\Large+$}
              
              \put(265,66){$g(t)$}
              \put(265,60){\vector(1,0){20}}
              \put(0,20){\sigb}
\end{picture}
}

\def\sigb{\setlength{\unitlength}{0.46pt}
\begin{picture}(290,108)
\thinlines    \put(10,26){\vector(1,0){260}}
              \put(10,12){\vector(0,1){88}}
              
              \put(20,27){\vector(0,1){34}}
              \put(40,27){\vector(0,1){14}}
              \put(60,27){\vector(0,1){54}}
              \put(80,27){\vector(0,1){31}}
              \put(100,27){\vector(0,1){46}}
              \put(120,27){\vector(0,1){40}}
              \put(140,27){\vector(0,1){48}}
              \put(160,27){\vector(0,1){34}}
              \put(180,27){\vector(0,1){14}}
              \put(200,27){\vector(0,1){31}}
              \put(220,27){\vector(0,1){46}}
              \put(240,27){\vector(0,1){40}}
              
              \put(270,14){$t$}
              %\put(22,90){$s(t)$}
              \put(15,10){$1$}
              \put(15,63){$\red{f_1}$}
              \put(135,10){$n$}
              \put(135,68){$\red{f_n}$}
              \put(235,10){$N$}
              \put(235,68){$\red{f_N}$}

              %\put(60,10){$\Delta t$}
\end{picture}
}

\def\sigbr{\setlength{\unitlength}{0.46pt}
\begin{picture}(290,108)
\thinlines    \put(10,26){\vector(1,0){260}}
              \put(10,12){\vector(0,1){88}}
              
              \put(20,27){\vector(0,1){34}}
              \put(40,27){\vector(0,1){14}}
              \put(60,27){\vector(0,1){54}}
              \put(80,27){\vector(0,1){31}}
              \put(100,27){\vector(0,1){46}}
              \put(120,27){\vector(0,1){40}}
              \put(140,27){\vector(0,1){48}}
              \put(160,27){\vector(0,1){34}}
              \put(180,27){\vector(0,1){14}}
              \put(200,27){\vector(0,1){31}}
              \put(220,27){\vector(0,1){46}}
              \put(240,27){\vector(0,1){40}}
              \put(270,14){$t$}
              %\put(22,90){$s(t)$}
              \put(15,10){$1$}
              \put(15,63){$\red{f_1}$}
              \put(135,10){$n$}
              \put(135,68){$\red{f_n}$}
              \put(235,10){$N$}
              \put(235,68){$\red{f_N}$}

              \put(60,10){$\red{\Delta t}$}
\end{picture}
}

\def\modelf{\tt\setlength{\unitlength}{0.92pt}
\begin{picture}(250,106)
\thinlines    \put(20,70){$s(t)=\sum_n \rfn \delta(t-n\red{\Delta t})$}
              \put(105,60){\vector(1,0){50}}
              \put(154,52){\framebox(50,16){$\Nc(t|0,\red{v})$}}
              
              \put(205,75){$g_{\rfb,\rthetab}(t)$}
              \put(204,60){\vector(1,0){33}}
              
              \put(252,85){$\epsilon(t)$}
              \put(250,95){\vector(0,-1){20}}
              \put(251,60){\circle{24}}
              \put(247,58){$\Large+$}
              
              \put(265,66){$g(t)$}
              \put(265,60){\vector(1,0){20}}
              \put(0,20){\sigbr}
\end{picture}
}

\def\sig{\tt\setlength{\unitlength}{1.38pt}
\begin{picture}(290,108)
\thinlines    %\put(179,83){$s_K(t)$}
              %\put(123,83){$s_k(t)$}
              %\put(70,83){$s_2(t)$}
              %\put(36,83){$s_1(t)$}
              \put(10,26){\vector(1,0){260}}
              \put(48,27){\vector(0,1){34}}
              \put(16,12){\vector(0,1){88}}
              \put(79,27){\vector(0,1){54}}
              \put(102,27){\vector(0,1){31}}
              \put(130,27){\vector(0,1){46}}
              \put(188,26){\vector(0,1){40}}
              \put(262,14){$t$}
              \put(22,90){$g(t)$}
              \put(182,16){$t_K$}
              \put(195,63){$a_K$}
              \put(125,15){$t_k$}
              \put(137,68){$a_k$}
              \put(75,14){$t_2$}
              \put(84,73){$a_2$}
              \put(43,15){$t_1$}
              \put(54,56){$a_1$}
              \multiput(150,46)(8,0){3}{\circle*{4}}
\end{picture}
}

\def\decgb{\tt\setlength{\unitlength}{0.92pt}
\begin{picture}(363,122)
\thinlines    \put(248,66){\vector(1,0){14}}
              \put(215,57){\framebox(33,18){$h(t)$}}
              \put(288,66){\vector(1,0){22}}
              \put(270,64){$\large\Sigma$}
              \put(275,67){\circle{26}}
              \put(275,102){\vector(0,-1){20}}
              \put(280,94){$b(t)$}
              \put(296,75){$y(t)$}
              \multiput(100,35)(0,8){3}{\circle*{4}}
              \put(194,72){$x(t)$}
              \put(193,66){\vector(1,0){23}}
              \put(176,61){$\large\Sigma$}
              \put(181,65){\circle{26}}
              \put(80,92){\framebox(43,18){$a_1$}}
              \put(80,58){\framebox(43,18){$a_2$}}
              \put(79,10){\framebox(43,18){$a_K$}}
              \put(123,66){\vector(1,0){45}}
              \put(123,101){\vector(4,-3){44}}
              \put(122,18){\vector(1,1){44}}
              \put(55,101){\vector(1,0){23}}
              \put(55,66){\vector(1,0){23}}
              \put(55,19){\vector(1,0){23}}
              \put(10,104){$g_1(t-t_1)$}
              \put(10,69){$g_2(t-t_2)$}
              \put(10,22){$g_K(t-t_k)$}
\end{picture}
}

\def\decgc{\tt\setlength{\unitlength}{0.92pt}
\begin{picture}(287,68)
\thinlines    \put(36,20){\vector(1,0){23}}
              \put(101,20){\vector(1,0){23}}
              \put(167,20){\vector(1,0){16}}
              \put(124,12){\framebox(43,18){$h(t)$}}
              \put(210,20){\vector(1,0){23}}
              \put(192,20){$\large\Sigma$}
              \put(196,23){\circle{26}}
              \put(196,57){\vector(0,-1){20}}
              \put(200,49){$b(t)$}
              \put(218,30){$y(t)$}
              \put(15,20){$s(t)$}
              \put(101,32){$x(t)$}
              \put(59,11){\framebox(43,18){$g(t)$}}
\end{picture}
}

\def\sigd{
\begin{picture}(290,108)
\thinlines    \put(10,26){\vector(1,0){260}}
              \put(48,27){\vector(0,1){34}}
              \put(16,12){\vector(0,1){88}}
              \put(79,27){\vector(0,1){54}}
              \put(102,27){\vector(0,1){31}}
              \put(130,27){\vector(0,1){46}}
              \put(188,26){\vector(0,1){40}}
              \put(262,14){$t$}
              \put(22,90){$g(t)$}
              \put(182,16){$t_K$}
              \put(195,63){$a_K$}
              \put(125,15){$t_k$}
              \put(137,68){$a_k$}
              \put(75,14){$t_2$}
              \put(84,73){$a_2$}
              \put(43,15){$t_1$}
              \put(54,56){$a_1$}
              \multiput(150,46)(8,0){3}{\circle*{4}}
\end{picture}
}

\def\wt#1{\widetilde{#1}}
\def\Thetab{\bm{\Theta}}
\def\Thetabh{\widehat{\Thetab}}
\def\abh{\widehat{\ab}}
\def\kbt{\tilde{\kb}}
\def\kt{\tilde{k}}
\def\gammat{\tilde{\gamma}}
\def\Sigmat{\tilde{\Sigma}}
\def\etat{\tilde{\eta}}

\def\rHb{\red{\Hb}}
\def\rFb{\red{\Fb}}

\def\wt#1{\widetilde{#1}}
\def\Thetab{\bm{\Theta}}
\def\Thetabh{\widehat{\Thetab}}
\def\abh{\widehat{\ab}}
\def\kbt{\tilde{\kb}}
\def\kt{\tilde{k}}
\def\gammat{\tilde{\gamma}}
\def\Sigmat{\tilde{\Sigma}}
\def\etat{\tilde{\eta}}
\def\zetat{\tilde{\zeta}}
\def\Mt{\tilde{M}}
\def\Mh{\hat{M}}
\def\Nt{\tilde{N}}
\def\atk{{\tilde{a}_k}}
\def\ztk{{\tilde{z}_k}}

\def\rh{\red{h}}
\def\rvbe{\rvb_{\epsilon}}
\def\rvei{\rv_{\epsilon_i}}
\def\rVbe{\rVb_{\epsilon}}
\def\rVbeh{\red{\Vbh}_{\epsilon}}
\def\vbh{\hat{\vb}}
\def\rVbfh{\red{\Vbh}_f}
\def\rvbeh{\rvbh_{\epsilon}}
\def\rvbet{\rvbt_{\epsilon}}
\def\rvbfh{\rvbh_f}

\def\rvbf{\rvb_f}
\def\rvfj{\rv_{f_j}}
\def\rVbf{\red{\Vb}_f}

\def\alphaez{\alpha_{\epsilon_0}}
\def\betaez{\beta_{\epsilon_0}}
\def\alphafz{\alpha_{f_0}}
\def\betafz{\beta_{f_0}}

\def\wh#1{\widehat{#1}}
\def\disp#1{{\displaystyle #1}}

\def\ER{\mbox{I\kern-.25em R}}
\def\EC{\mbox{C\kern-.8em C}}
\def\EZ{\mbox{Z\kern-.55em Z}}
\def\EN{\mbox{N\kern-.8em N}}

\def\bm#1{\mbox{\boldmath $#1$}}
\def\sb{{\bm s}}
\def\ub{{\bm u}}
\def\xb{{\bm x}}
\def\yb{{\bm y}}
\def\db{{\bm{d}}}
\def\Ab{{\bm A}}
\def\Bb{{\bm B}}
\def\Fb{{\bm F}}
\def\Rb{{\bm R}}
\def\Sb{{\bm S}}
\def\Ub{{\bm U}}

\def\thetab{\bm{\theta}}
\def\phib{\bm{\phi}}
\def\lambdab{\bm{\lambda}}
\def\Lambdab{\bm{\Lambda}}
\def\Sigmab{\bm{\Sigma}}
\def\lra{\longrightarrow}
\def\intg{\int\kern-1.1em\int}
\def\intd{\int\kern-.8em\int}

\def\apriori{{\em a priori} }
\def\aposteriori{{\em a posteriori} }

\def\d#1{\,\mbox{d}#1}
\def\esp#1{\mbox{E}\left\{ #1 \right\}}
\def\espx#1#2{\mbox{E}_{#1}\left\{ #2 \right\}}
\def\expf#1{\exp\left[ {#1} \right]}
\def\dpdx#1#2{\frac{\partial #1}{\partial #2}}
\def\dpdxd#1#2{\frac{\partial^2 #1}{\partial #2^2}}

\def\ent#1{\hbox{H}\left[#1\right]}
\def\dent#1{\delta\hbox{H}\left[#1\right]}
\def\rent#1{\hbox{D}\left[#1\right]}
\def\kullback#1{\hbox{K}\left[#1\right]}
\def\pent#1{\hbox{PE}\left[#1\right]}
\def\mdiv#1{\hbox{J}\left[#1\right]}
\def\infmut#1{\hbox{I}\left[#1\right]}
\def\idisc#1{\hbox{ID}\left[#1\right]}
\def\j{\mbox{j}}

\def\pxtheta{p(x | \thetab)}
\def\pxthetas{p(x | \thetab^*)}
\def\pxthetasd{p(x | \thetab^*+\Delta\thetab)}

\def\tr#1{\hbox{tr}\left(#1\right)}
\def\det#1{\hbox{det}\left(#1\right)}
%\def\det#1{\left| #1\right| }


\def\ieeeSSC{IEEE Transactions on Systems Science and Cybernetics}
\def\ieeeSP{IEEE Transactions on Signal Processing}			% 1.234
\def\ieeeP{Proceedings of the IEEE}					% ?
\def\ieeeIT{IEEE Transactions on Information Theory}			% 1.971
\def\TS{Traitement du Signal}						% ?
\def\siamCO{SIAM Journal of Control}					% 0.968
\def\AISM{Annals of Institute of Statistical Mathematics}		% 0.175
\def\ieeeASSP{IEEE Transactions on Acoustics Speech and Signal Processing}% ?
\def\ieeeAC{IEEE Transactions on Automatic and Control}			% 0.867

\def\jan{janvier\xspace}
\def\feb{f\'evrier\xspace}
\def\mar{mars\xspace}
\def\apr{avril\xspace}
\def\may{mai\xspace}
\def\jun{juin\xspace}
\def\jul{juillet\xspace}
\def\aug{ao\^ut\xspace}
\def\sep{septembre\xspace}
\def\oct{octobre\xspace}
\def\nov{novembre\xspace}
\def\dec{d\'ecembre\xspace}
%
\def\Jan{January\xspace}	
\def\Feb{February\xspace}
\def\Mar{March\xspace}
\def\Apr{April\xspace}
\def\May{May\xspace}
\def\Jun{June\xspace}
\def\Jul{July\xspace}
\def\Aug{August\xspace}
\def\Sep{September\xspace}
\def\Oct{October\xspace}
\def\Nov{November\xspace}
\def\Dec{December\xspace}


\def\espq#1{\left<#1\right>_q}

\def\rZbe{\rZb_{\epsilon}}
\def\nubt{\widetilde{\nub}}

\def\rVbf{\rVb_{f}}
\def\rvbf{\rvb_{f}}
\def\rvfj{\red{v}_{f_j}}
\def\rvbhe{\rvbh_{\epsilon}}
\def\rvbhf{\rvbh_{f}}
\def\bsplit{\begin{split}}
\def\esplit{\end{split}}
\def\alphaei{\alpha_{\epsilon_i}}
\def\alphafj{\alpha_{f_j}}
\def\betaei{\beta_{\epsilon_i}}
\def\betafj{\beta_{f_j}}

\def\bgbh{\widehat{\bgb}}
\def\rfh{\widehat{\rf}}
\def\rFh{\widehat{\rF}}
\def\rc{\red{r}}
\def\rch{\widehat{\rc}}
\def\partialx{\frac{\partial }{\partial x}}
\def\partialy{\frac{\partial }{\partial y}}
\def\partialr{\frac{\partial }{\partial r}}
\def\partialxd{\frac{\partial^2 }{\partial x^2}}
\def\partialyd{\frac{\partial^2 }{\partial y^2}}
\def\partialrd{\frac{\partial^2 }{\partial r^2}}
\def\cosphi{\cos(\phi)}
\def\sinphi{\sin(\phi)}
\def\sumk{\sum_{k=1}^K}
\def\sumj{\sum_{j=1}^N}
\def\sumi{\sum_{i=1}^M}
\def\summ{\sum_{m=1}^M}
\def\sumn{\sum_{n=1}^N}
\def\summn{\sum_{m=1}^M\sum_{n=1}^N}

\def\df{\dot{f}}
\def\ddf{\ddot{f}}

\def\rf{\red{f}}
\def\rdf{\red{\df}}
\def\rddf{\red{\ddf}}

\def\rfb{\red{\fb}}
\def\rdfb{\red{\dot{\fb}}}
\def\rddfb{\red{\ddot{\fb}}}

\def\bdg{\blue{\dot{g}}}
\def\bddg{\blue{\ddot{g}}}

\def\bgb{\blue{\gb}}
\def\bdg{\blue{\dot{g}}}

\def\bdgb{\blue{\dot{\gb}}}
\def\bddgb{\blue{\ddot{\gb}}}

\def\epsilonbd{\dot{\epsilonb}}
\def\epsilonbdd{\ddot{\epsilonb}}

\def\rdfbh{\widehat{\rdfb}}
\def\rddfbh{\widehat{\rddfb}}

\def\rqh{\red{\widehat{q}}}
\def\rdfh{\red{\widehat{\dot{f}}}}
\def\rddfh{\red{\widehat{\ddot{f}}}}

\def\vek{v_{\epsilon_k}}
\def\rveih{\widehat{\rve}_i}
\def\rvfjh{\widehat{\rvf}_j}

\def\alphaxiz{{\alpha_{\xi_0}}}
\def\betaxiz{{\beta_{\xi_0}}}
\def\alphazz{{\alpha_{z_0}}}

\def\betazz{{\beta_{z_0}}}
\def\rVbz{{\rVb_z}}
\def\rvbz{{\rvb_z}}
\def\rvxi{{\rv_\xi}}
\def\rvzj{{\rv_{z_j}}}
\def\rvxih{{\widehat{\rv}_\xi}}
\def\rvbzh{{\widehat{\rvb}_z}}
\def\rvzjh{{\widehat{\rv}_{z_j}}}

\def\alphae{{\alpha_\epsilon}}

\def\alphaet{{\widetilde{\alpha}_\epsilon}}
\def\alphaft{{\widetilde{\alpha}_f}}
\def\betae{{\beta_\epsilon}}
\def\betaet{{\widetilde{\beta}_\epsilon}}
\def\betaft{{\widetilde{\beta}_f}}
\def\rfih{\hat{\rf}_i}
\def\rfbk{\rfb^{(k)}}
\def\rfbkp{\rfb^{(k+1)}}

\def\rmh{\hat{\red{m}}}

\def\rmk{{\red{m}_k}}
\def\rmkh{{\hat{\red{m}}_k}}
\def\rvk{{\red{v}_k}}
\def\rvkh{{\hat{\red{v}}_k}}
\def\rak{{\red{a}_k}}
\def\rakh{{\hat{\red{a}}_k}}

\def\rvh{\hat{\red{v}}}
\def\rveh{\hat{\rve}}

\def\rmt{\tilde{\red{m}}}
\def\rvt{\tilde{\red{v}}}
\def\rvet{\tilde{\rve}}
\def\rveih{\red{\hat{v}}_{\epsilon_i}}

\def\rveb{\red{\vb_{\epsilon}}}
\def\rvebh{\red{\vbh_{\epsilon}}}

%---------------------------------------------------------------
\def\blocgi{\begin{picture}(80,50)
  \put(60,40){\makebox(0,0){$\red{m}$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\blue{g}_i$}}
  \put(20,0){\circle{20}}
  \put(20,0){\makebox(0,0){$\epsilon_i$}}
  \put(30,0){\vector(1,0){20}}
\end{picture}
}
\def\blocgfi{\begin{picture}(80,50)
  \put(60,40){\makebox(0,0){$\rf_i$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\blue{g}_i$}}
  \put(20,0){\circle{20}}
  \put(20,0){\makebox(0,0){$\epsilon_i$}}
  \put(30,0){\vector(1,0){20}}
\end{picture}
}
\def\blocghfi{\begin{picture}(80,50)
  \put(60,40){\makebox(0,0){$\rf_i$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(65,20){\makebox(0,0){$h$}}
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\blue{g}_i$}}
  \put(20,0){\circle{20}}
  \put(20,0){\makebox(0,0){$\epsilon_i$}}
  \put(30,0){\vector(1,0){20}}
\end{picture}
}
\def\blocgie{\begin{picture}(80,50)
  \put(60,40){\makebox(0,0){$\red{m}$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\blue{g}_i$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilon_i$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocgievei{\begin{picture}(80,50)
  \put(60,40){\makebox(0,0){$\red{m}$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\blue{g}_i$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilon_i$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rvei$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocfgie{\begin{picture}(80,100)
  \put(60,40){\makebox(0,0){$\rf_i$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(65,20){\makebox(0,0){$\blue{h}$}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\blue{g}_i$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilon_i$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocvfgie{\begin{picture}(80,100)
  \put(60,80){\makebox(0,0){$\rv_i$}}
  \put(60,80){\circle{20}}
  \put(60,70){\vector(0,-1){20}}
  
  \put(60,40){\makebox(0,0){$\rf_i$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(65,20){\makebox(0,0){$\blue{h}$}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\blue{g}_i$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilon_i$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocvfhgie{\begin{picture}(80,100)
  \put(60,80){\makebox(0,0){$\rv_i$}}
  \put(60,80){\circle{20}}
  \put(60,70){\vector(0,-1){20}}
  
  \put(60,40){\makebox(0,0){$\rf_i$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  
  \put(30,30){\circle{20}}
  \put(30,30){\makebox(0,0){$\red{h}$}}
  \put(38,22){\vector(1,-1){15}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\blue{g}_i$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilon_i$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocvfhgiei{\begin{picture}(80,100)
  \put(60,80){\makebox(0,0){$\rv_i$}}
  \put(60,80){\circle{20}}
  \put(60,70){\vector(0,-1){20}}
  
  \put(60,40){\makebox(0,0){$\rf_i$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  
  \put(30,30){\circle{20}}
  \put(30,30){\makebox(0,0){$\red{h}$}}
  \put(38,22){\vector(1,-1){15}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\blue{g}_i$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilon_i$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rvei$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocfgHe{\begin{picture}(80,100)
  \put(60,40){\makebox(0,0){$\rfb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(65,20){\makebox(0,0){$\blue{\Hb}$}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocvfgHe{\begin{picture}(80,100)
  \put(60,80){\makebox(0,0){$\rvb$}}
  \put(60,80){\circle{20}}
  \put(60,70){\vector(0,-1){20}}
  
  \put(60,40){\makebox(0,0){$\rfb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(65,20){\makebox(0,0){$\bHb$}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocvfgHei{\begin{picture}(80,100)
  \put(60,80){\makebox(0,0){$\rvb$}}
  \put(60,80){\circle{20}}
  \put(60,70){\vector(0,-1){20}}
  
  \put(60,40){\makebox(0,0){$\rfb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(65,20){\makebox(0,0){$\bHb$}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rvei$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocvfHge{\begin{picture}(80,100)
  \put(60,80){\makebox(0,0){$\rvb$}}
  \put(60,80){\circle{20}}
  \put(60,70){\vector(0,-1){20}}
  
  \put(60,40){\makebox(0,0){$\rfb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  
  \put(30,30){\circle{20}}
  \put(30,30){\makebox(0,0){$\rHb$}}
  \put(38,22){\vector(1,-1){15}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocvfHgei{\begin{picture}(80,100)
  \put(60,80){\makebox(0,0){$\rvb$}}
  \put(60,80){\circle{20}}
  \put(60,70){\vector(0,-1){20}}
  
  \put(60,40){\makebox(0,0){$\rfb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  
  \put(30,30){\circle{20}}
  \put(30,30){\makebox(0,0){$\rHb$}}
  \put(38,22){\vector(1,-1){15}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rvei$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocvhFge{\begin{picture}(80,100)
  \put(60,80){\makebox(0,0){$\rvb$}}
  \put(60,80){\circle{20}}
  \put(60,70){\vector(0,-1){20}}
  
  \put(60,40){\makebox(0,0){$\rhb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  
  \put(30,30){\circle{20}}
  \put(30,30){\makebox(0,0){$\bFb$}}
  \put(38,22){\vector(1,-1){15}}

  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocvhFgei{\begin{picture}(80,100)
  \put(60,80){\makebox(0,0){$\rvb$}}
  \put(60,80){\circle{20}}
  \put(60,70){\vector(0,-1){20}}
  
  \put(60,40){\makebox(0,0){$\rhb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  
  \put(30,30){\circle{20}}
  \put(30,30){\makebox(0,0){$\bFb$}}
  \put(38,22){\vector(1,-1){15}}

  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rvei$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blochFge{\begin{picture}(80,40)
  \put(60,40){\makebox(0,0){$\rhb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  
  \put(30,30){\circle{20}}
  \put(30,30){\makebox(0,0){$\bFb$}}
  \put(38,22){\vector(1,-1){15}}

  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blochFgei{\begin{picture}(80,40)
  \put(60,40){\makebox(0,0){$\rhb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  
  \put(30,30){\circle{20}}
  \put(30,30){\makebox(0,0){$\bFb$}}
  \put(38,22){\vector(1,-1){15}}

  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rvei$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocfHge{\begin{picture}(80,40)  
  \put(60,40){\makebox(0,0){$\bfb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  
  \put(30,30){\circle{20}}
  \put(30,30){\makebox(0,0){$\rHb$}}
  \put(38,22){\vector(1,-1){15}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocfHgei{\begin{picture}(80,40)  
  \put(60,40){\makebox(0,0){$\bfb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  
  \put(30,30){\circle{20}}
  \put(30,30){\makebox(0,0){$\rHb$}}
  \put(38,22){\vector(1,-1){15}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rvei$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}
\def\blocFgHe{\begin{picture}(80,40)
  \put(60,40){\makebox(0,0){$\bfb$}}
  \put(60,40){\circle{20}}
  \put(60,30){\vector(0,-1){20}}
  \put(65,20){\makebox(0,0){$\blue{\rHb}$}}
  
  \put(60,0){\circle{20}}
  \put(60,0){\makebox(0,0){$\bgb$}}
  \put(30,0){\circle{20}}
  \put(30,0){\makebox(0,0){$\epsilonb$}}
  \put(40,0){\vector(1,0){10}}
  \put(0,0){\circle{20}}
  \put(0,0){\makebox(0,0){$\rve$}}
  \put(10,0){\vector(1,0){10}}
\end{picture}
}

\def\ftrfi{\bg(r,\phi)}
\def\wth{\widehat{\tilde{h}}}
\def\varx#1#2{\mbox{Var}_{#1}\left\{#2\right\}}
\def\rvbxi{\rvb_{\xi}}
\def\rVbxi{\rVb_{\xi}}
\def\rvbxih{\rvbh_{\xi}}

\def\repsilon{\red{\epsilon}}


\def\vzj{v_{z_j}}
\def\vxij{v_{\xi_j}}
\def\vei{v_{\epsilon_i}}

\def\vzjh{\widehat{v}_{z_j}}
\def\vxijh{\widehat{v}_{\xi_j}}
\def\veih{\widehat{v}_{\epsilon_i}}

\def\vbeh{\widehat{\vb}_{\epsilon}}
\def\vbxih{\widehat{\vb}_{\xi}}
\def\vbzh{\widehat{\vb}_{z}}

\def\Vbeh{\widehat{\Vb}_{\epsilon}}
\def\Vbxih{\widehat{\Vb}_{\xi}}
\def\Vbzh{\widehat{\Vb}_{z}}

\def\Ybeh{\widehat{\Yb}_{\epsilon}}
\def\Ybxih{\widehat{\Yb}_{\xi}}
\def\Ybzh{\widehat{\Yb}_{z}}

\def\vf{v_f}
\def\vbe{\vb_{\epsilon}}
\def\vbz{\vb_z}
\def\vxi{v_{\xi}}
\def\vbxi{\vb_{\xi}}
\def\Vbe{\Vb_{\epsilon}}
\def\Vbxi{\Vb_{\xi}}
\def\Vbz{\Vb_z}

\def\half{\frac{1}{2}}

\def\dpdx#1#2{\frac{\partial {#1}}{\partial {#2}}}
\def\dpdxd#1#2{\frac{\partial^2 {#1}}{\partial {#2}^2}}
\def\dpdxdy#1#2#3{{{\partial ^2 {#1}}\over{\partial {#2} \partial {#3}}}}

\def\KL#1#2{\mbox{KL}\left[#1 : #2\right]}
\def\Covx#1#2{\mbox{Cov}_{#1}(#2)}
\def\braket#1#2{<{#1}(#2)>}

\def\rlambdab{\red{\lambdab}}
\def\bve{\blue{\ve}}
\def\ralphafjt{\red{\tilde{\alpha}_{f_j}}}
\def\rbetafjt{\red{\tilde{\beta}_{f_j}}}
\def\rSigmabt{\red{\tilde{\Sigmab}}}
\def\rfjt{\red{\tilde{f_j}}}
\def\zetab{\bm{\zeta}}
\def\bvxi{\blue{v_\xi}}
\def\bgamma{\blue{\gamma}}
\def\rgamma{\red{\gamma}}
\def\alphagamz{\alpha_{\gamma_0}}
\def\betagamz{\beta_{\gamma_0}}
\def\alphazetaz{\alpha_{\zeta_0}}
\def\betazetaz{\beta_{\zeta_0}}

\def\bvf{\blue{v_f}}
\def\bvzeta{\blue{v_\zeta}}
\def\rgb{\red{\gb}}
\def\rvxii{\red{v_{\xi_i}}}
\def\rvzeta{\red{v_{\zeta}}}


%------------- package tikz -------------------
\usepackage{tikz,mathpazo}
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{positioning,shapes,shadows,arrows}
\usetikzlibrary{mindmap,backgrounds}
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=1.5cm, minimum height=0.5cm,text centered, draw=black]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=1.5cm, minimum height=0.6cm, text centered, draw=black]
\tikzstyle{process} = [rectangle, minimum width=1cm, minimum height=0.5cm, text centered, draw=black]
\tikzstyle{note} = [text centered]
\tikzstyle{decision} = [diamond, minimum width=1.5cm, minimum height=0.3cm, text centered, draw=black]
\tikzstyle{arrow} = [thick,->,>=stealth]

\def\blambda{\blue{\lambda}}
\def\blambdab{\blue{\lambdab}}


\def\fxy{f(x,y)}
\def\afxy{a\left(f(x,y)\right)}

\def\hxy{h(x,y)}
\def\gxy{g(x,y)}

\def\gt{\widetilde{g}}
\def\ft{\widetilde{f}}
\def\htxy{\widetilde{h}(x,y)}
\def\htzero{\widetilde{h}_0}
\def\htone{\widetilde{h}_1}
\def\httwo{\widetilde{h}_2}

\def\hdxy{h_d(x,y)}
\def\gdxy{g_d(x,y)}

\def\exy{\epsilon(x,y)}
\def\nxy{n(x,y)}
\def\rxy{r(x,y)}

\def\dxy{d(x,y)}
\def\dhxy{d_h(x,y)}
\def\dfxy{d_f(x,y)}

\def\fhxy{\hat{f}(x,y)}
\def\ghxy{\hat{f}(x,y)}
\def\ehxy{\hat{\epsilon}(x,y)}
\def\nhxy{\hat{n}(x,y)}

\def\ftuv{\widetilde{f}(u,v)}
\def\htuv{\widetilde{h}(u,v)}
\def\gtuv{\widetilde{g}(u,v)}
\def\rtuv{\widetilde{r}(u,v)}
\def\ntuv{\widetilde{n}(u,v)}
\def\dtuv{\widetilde{d}(u,v)}
\def\dhtuv{\widetilde{d}_h(u,v)}
\def\dftuv{\widetilde{d}_f(u,v)}

\def\htcuv{\widetilde{h}^*(u,v)}
\def\ftcuv{\widetilde{f}^*(u,v)}

\def\ftuv{\widetilde{f}(u,v)}
\def\htuv{\widetilde{h}(u,v)}
\def\etuv{\widetilde{\epsilon}(u,v)}

\def\ftcuv{\widetilde{f}^*(u,v)}
\def\htcuv{\widetilde{h}^*(u,v)}
\def\etcuv{\widetilde{\epsilon}^*(u,v)}

\def\fhtuv{\widehat{\widetilde{f}}(u,v)}
\def\hhtuv{\widehat{\widetilde{h}}(u,v)}

\def\fhtxy{\widehat{\widetilde{f}}(x,y)}
\def\hhtxy{\widehat{\widetilde{h}}(x,y)}

\def\fhtcuv{\widehat{\widetilde{f}}^*(u,v)}
\def\hhtcuv{\widehat{\widetilde{h}}^*(u,v)}
\def\ghtcuv{\widehat{\widetilde{g}}^*(u,v)}

\def\htzerouv{\widetilde{h}_0(u,v)}
\def\htoneuv{\widetilde{h}_1(u,v)}
\def\httwouv{\widetilde{h}_2(u,v)}
\def\htzerocuv{\widetilde{h}_0^*(u,v)}
\def\htonecuv{\widetilde{h}_1^*(u,v)}
\def\httwocuv{\widetilde{h}_2^*(u,v)}
\def\gtoneuv{\widetilde{g}_1(u,v)}
\def\gttwouv{\widetilde{g}_2(u,v)}

\def\ftuvk{\widetilde{f}^{(k)}(u,v)}
\def\htuvk{\widetilde{h}^{(k)}(u,v)}

\def\fhxyk{\widehat{f}^{(k)}(x,y)}
\def\hhxyk{\widehat{h}^{(k)}(x,y)}
\def\fhxykp{\widehat{f}^{(k+1)}(x,y)}
\def\hhxykp{\widehat{h}^{(k)}(x,y)}

\def\fhk{\widehat{f}^{(k)}}
\def\hhk{\widehat{h}^{(k)}}
\def\fhkp{\widehat{f}^{(k+1)}}
\def\hhkp{\widehat{h}^{(k)}}

\def\fxyk{f^{(k)}(x,y)}
\def\fxykp{f^{(k+1)}(x,y)}

\def\fkxy{f^{(k)}(x,y)}
\def\fkpxy{f^{(k+1)}(x,y)}

\def\ftuvkp{\widetilde{f}^{(k+1)}(u,v)}
\def\htuvkp{\widetilde{h}^{(k+1)}(u,v)}

\def\hktuv{\widetilde{h}_k(u,v)}
\def\gktuv{\widetilde{g}_k(u,v)}

\def\bfxy{\blue{f}(x,y)}
\def\bhxy{\blue{h}(x,y)}
\def\bgxy{\blue{g}(x,y)}

\def\rfxy{\red{f}(x,y)}
\def\rhxy{\red{h}(x,y)}

\def\rftuv{\widetilde{\red{f}}(u,v)}
\def\rhtuv{\widetilde{\red{h}}(u,v)}

\def\bgtuv{\widetilde{\blue{g}}(u,v)}

\def\alphabh{\widehat{\alphab}}

\def\dfdx#1#2{\frac{\partial #1}{\partial #2}}

\def\zxy{z(x,y)}
\def\Txy{T(x,y)}
\def\fxy{f(x,y)}
\def\gzxy{g_0(x,y)}
\def\gxy{g(x,y)}
\def\phixy{\phi(x,y)}
\def\exy{e(x,y)}
\def\epsxy{\epsilon(x,y)}

\def\zhxy{\hat{z}(x,y)}
\def\Thxy{\hat{T}(x,y)}
\def\gzhxy{\hat{g}_0(x,y)}
\def\fhxy{\hat{f}(x,y)}
\def\phihxy{\hat{\phi}(x,y)}
\def\epshxy{\hat{\epsilon}(x,y)}


